mLoRA: Fine-Tuning LoRA Adapters via Highly-Efficient Pipeline Parallelism in Multiple GPUs

Transformer-based, pre-trained large language models (LLMs) have demonstrated outstanding performance across diverse domains, particularly in the emerging {\em pretrain-then-finetune} paradigm. Low-Rank Adaptation (LoRA), a parameter-efficient fine-tuning method, is commonly used to adapt a base LLM to multiple downstream tasks. Further, LLM platforms enable developers to fine-tune multiple models and develop various domain-specific applications simultaneously. However, existing model parallelism schemes suffer from high communication overhead and inefficient GPU utilization when training multiple LoRA tasks across GPUs and machines. In this paper, we present mLoRA, a parallelism-efficient fine-tuning system designed for training multiple LoRA across GPUs and machines. mLoRA introduces a novel LoRA-aware pipeline parallelism scheme that efficiently pipelines independent LoRA adapters and their distinct fine-tuning stages across GPUs and machines, along with a new LoRA-efficient operator to enhance GPU utilization during pipelined LoRA training. Our extensive evaluation shows that mLoRA can significantly reduce average fine-tuning task completion time, e.g., by 30\%, compared to state-of-the-art methods like FSDP. More importantly, mLoRA enables simultaneous fine-tuning of larger models, e.g., two Llama-2-13B models on four NVIDIA RTX A6000 48GB GPUs, which is not feasible for FSDP due to high memory requirements. Hence, mLoRA not only increases fine-tuning efficiency but also makes it more accessible on cost-effective GPUs. mLoRA has been deployed in AntGroup's production environment.

==> OLDVER/OLDVER/chapters/I._Introduction.tex <==
\begin{figure*}[ht]
    \centering
    %\vspace{-10pt}
    \includegraphics[width=0.9\linewidth]{pics/early_stop_example.pdf}
    %\vspace{-1em}
    \caption{An example of adaptive job scheduling.}
    \label{fig:early-stop}
    %\vspace{-0.5em}
\end{figure*}

\begin{figure}[t]
    \centering 
    \begin{minipage}{1.6in}
    \subfigure[]{
        \centering 
        \includegraphics[width=1\linewidth]{pics/pad.pdf}
        %\vspace{2em}
        \label{fig:pad}
    }
    \hfill
    \end{minipage}
    \begin{minipage}{1.7in}
    \subfigure[]{
        \centering    
        \includegraphics[width=1\linewidth]{pics/data_distribution.pdf}
        \label{fig:data_distribution}
    }
    \end{minipage}
    \caption{An example of a fused batch (the proportion of pad tokens is 25\%) and distribution of various datasets.}
    %\vspace{-2em}
\end{figure}
% Intro to the LLM background

% intro the llm and lora popularirty, and fine tune is very important topic

% introduces the mulit-Lora idea by sharing the memory 

% introduce this is not a trivial work 

% 1. padding issues and effective throughput  
% 2. OOM issues and dynamic number of jobs fine tuning in parallel
% 3. early stop issues in the model fine-tune 

 % therefore, our contributions

 % 1. throughput oriented padding 
 % 2. job resource usage modeling and prediction
 % 3. early stop modeling and policy
 % 4. adaptive multi-lora jobs scheduling algorithm 

%In recent years, generative language models based on the Transformer\cite{vaswani2023attention} architecture, also known as large language models (LLMs), have demonstrated formidable capabilities in a broad spectrum of nature language processing (NLP) tasks and the processing of multi-modal data. Currently, prominent pre-trained models include GPT, LLaMA, ChatGLM, and others.
%GPT, LLaMA add reference here
%Large Language Models (LLMs) have made a significant impact across a wide range of  on modern applications, spanning from natural language processing to a broader spectrum of tasks (OpenAI, 2023; Touvron et al., 2023b; Alayrac et al., 2022). %These models showcase exceptional performance in various domains, especially when {\em fine-tuned} for specialized tasks (Kenton Toutanova, 2019; Houlsby et al., 2019; Ouyang et al., 2022). 
Large language models (LLMs) have a significant impact on modern applications, expanding from natural language processing to a broader spectrum of domain-specific tasks, such as OpenAI-Chatgpt~\cite{openai-chatgpt}, fine-tuned LLMs~\cite{touvron2023llama,vicuna2023,fastchat,du2022glm,touvron2023llama}, and visual language models~\cite{alayrac2022flamingo,zhang2021vinvl}. To adapt an LLM to multiple downstream applications, a common practice is to {\em pre-train} the model on large datasets, followed by {\em fine-tuning} it for applications~\cite{brown2020language,devlin2018bert,houlsby2019parameter,ouyang2022training}.
%has given rise to numerous distinct versions of a pre-trained model. Each version is tailored to excel in specific tasks or domains, highlighting the versatility and effectiveness of LLMs in today's technological landscape.

Fine-tuning can be very expensive, typically requiring updates to all parameters of the pre-trained model (i.e., full-weight update), and the fine-tuned model may contain as many parameters as the pre-trained one~\cite{lv2023parameter}. To overcome this, Low-Rank Adaptation (LoRA)~\cite{hu2021lora} enables efficient fine-tuning of a pre-trained model by creating small LoRA modules for different tasks. It is achieved by freezing the pre-trained model and only updating low-rank additive matrices, with much fewer parameters (than the pre-trained one).

LoRA greatly reduces the computational resources, making the fine-tuning process feasible across various tasks.
%As the fine-tuning of a pre-trained model extends to encompass a broad spectrum of tasks, such as those found in personalized assistants, the associated costs for both training and serving the model can become considerably high. In addressing this challenge, various parameter-efficient fine-tuning methods have been developed. Among them, Low-Rank Adaptation (LoRA), introduced by Hu et al\cite{hu2021lora} in 2021, stands out. LoRA enables efficient fine-tuning by focusing on updating only low-rank additive matrices, rather than the entire set of model parameters. This approach significantly reduces the computational burden and resource requirements, making the fine-tuning process more efficient and manageable, especially when scaling across a wide array of tasks.i
For example, by the end of November 2023, thousands of LLaMA models~\cite{touvron2023llama} had been fine-tuned based on LoRA, accessible on the Hugging Face Hub~\cite{hugging-face}. Further, on the HuggingFace Leaderboard~\cite{open-llm-leaderboard}, 40\% of the top 20 language models feature fine-tuning of the LLaMA model using LoRA and/or its derivatives.
% we can say: 1. 1/2 chatglm based model in HF is LoRA based 2. 1/3 Baichuan or Qiwen is also LoRA based. 3. more information is better
As of November 10, 2023, the highest-ranking LoRA-based model, GodziLLa2-70B~\cite{godzilla2-70b}, is positioned 2nd, trailing the top-ranked LLM by only 1.67 points in the average performance evaluation score.
%The highest-ranking LoRA-based model is GodziLLa2-70B~\cite{godzilla2-70b}, positioned 2nd as of November 10, 2023, only 1.67 points behind the top-ranked LLM in the average score of performance evaluation.
% give more details here, this is danger
These practical applications show that LoRA is not only extensively used for fine-tuning tasks in LLMs but also achieves high model accuracy comparable to other (full-weight) fine-tuning methods.
%Additionally, to boost the performance of the LoRA approach, several derivative methods have been developed: QLoRA~\cite{dettmers2023qlora} backpropagates gradients through a frozen, 4-bit quantized pre-trained language model;
%into LoRA; 
%LoftQ~\cite{li2023loftq}
%a novel quantization framework that 
%simultaneously quantizes an LLM and finds a proper low-rank initialization for LoRA fine-tuning.
% we had better also introduce other LORA based approach like QloRA, o-LORA, etc. 

%LoRA's approach, focusing only on fine-tuning the adapter weights, has proven to be quite effective, achieving performance on par with full-weight fine-tuning methods; moreover, 
%redudent -- stated in the above paragraph #hui
The extremely lightweight nature of LoRA-based fine tuning further allows for training {\em multiple} LoRA modules on a \emph{single} commercial GPU. Intuitively, sharing a pre-trained model training among multiple training LoRA modules should bring the same benefits like reduced GPU memory usage and improved computation efficiency. However, a straightforward sharing approach -- e.g., by only swapping in/out LoRA modules while keeping the pre-trained model in GPU memory when training multiple LoRA jobs -- may introduce additional overheads, which could be suboptimal. Moreover, current LoRA-based fine-tuning systems, such as Alpaca-LoRA~\cite{alpaca-lora}, predominantly concentrate on optimizing single-job fine-tuning and have not thoroughly investigated efficient strategies for fine-tuning multiple jobs.
%\Lan{explain why existing methods fail in short words?}
%only focus on optimizing a single job.
%The substantial reduction in computational resources by LoRA further allows for fine-tuning of {\em multiple} LLMs on a {\em single} commercial GPU.
%such as the NVIDIA RTX A6000.

%With LoRA's efficient utilization of computational resources, it becomes feasible for individuals to train LLMs on a single commercial GPU like NVIDIA RTX A6000. Yet, even with this extensive research into fine-tuning methodologies, a crucial aspect remains unaddressed: the efficient fine-tuning of these variants on a single GPU setup. This particular challenge involves not just the aspect of model performance, but also the optimization of resource usage, especially in environments limited to a single GPU. Addressing this will be key in making fine-tuning processes more accessible and practical, especially for scenarios with resource constraints.

%Due to the substantial data and computational resources required for the pre-training process of large language models, fine-tuning is commonly employed to imbue pre-trained models with domain-specific knowledge. There are various fine-tuning methods, such as full parameter fine-tuning, P-Tuning, and notably, LoRA (Low-Rank Adaptation)\cite{hu2021lora}. Initially proposed by Microsoft in 2021, LoRA's key concept involves utilizing a separate low-rank parameter update matrix to represent the updates to the pre-trained model's parameters. This approach offers advantages such as conserving GPU memory during fine-tuning and representing fine-tuning results with smaller weights without sacrificing accuracy.
% do we need to emphasis that LoRA is good for individual to fine tune model on the commercial GPU like 4090 or others. 

%In this paper, we present {ASPEN}, a high-throughput framework designed for fine-tuning multiple LoRA LLMs on a single GPU. Aspen builds on top of a novel parallel fine-tuning approach to train multiple LoRA tasks concurrently by sharing pre-trained models. Regarding scheduling, Aspen integrates a fine-grained job-level scheduler to coordinate multiple LoRA tasks efficiently. ASPEN has addressed the following main challenges:

In this paper, we present ASPEN, a high-throughput fine-tuning framework designed for training multiple LoRA fine-tuning jobs on a single GPU. ASPEN builds on top of a novel parallel fine-tuning approach called {\em BatchFusion}, which enables the concurrent training of multiple LoRA fine-tuning jobs and the sharing of pre-trained models by fusing multiple input batches into a single batch. Allocating system resources efficiently for multiple jobs is a complex task. Therefore, ASPEN incorporates a fine-grained, efficient job-level scheduler for handling multiple LoRA jobs. ASPEN has successfully tackled the following key issues:
%\Hao{this seems a little trivial?} 
%Regarding scheduling, Aspen integrates a fine-grained job-level scheduler to coordinate multiple LoRA jobs efficiently. ASPEN has addressed the following main challenges:

%with low GPU memory usage and high computation efficiency. 
%In this paper, we investigate the efficiency of fine-tuning multiple LoRA adapters on a single GPU. Our observation is that the shared pre-trained model, which forms the foundation for numerous LoRA adapters, offers a significant potential to reduce the GPU memory usage and improves the computation efficiency. While incorporating batching into the pre-trained model is relatively straightforward since all fine-tuned models share the pre-trained model, extending batching to the adapters presents a challenge. 

% At first, we observed an uneven distribution of token lengths in the training dataset. Prior to training, we pre-allocated computing resources (primarily GPU memory) based on the maximum token length. However, the training dataset's uneven distribution led to suboptimal utilization of the reserved computing resources during the training process. To enhance the efficiency of resource utilization, we explored alternative approaches, particularly when resource utilization rates were low. One such approach involved reallocating unused computing resources to other jobs, facilitating parallel multi-job training.
% this is not clear: padding issues and effective throughput  

%While Batch Fusion enabled concurrent training effectively, it may lead to a higher proportion of padding tokens for alignment requirements.
%ASPEN fuses training data from multiple fine-tuning jobs into a single batch, enabling concurrent training of multiple LoRA modules with the same pre-trained model.\Lan{ASPEN fuses training data from multiple fine-tuning jobs into a single batch to enable multiple LoRA training, which can lead to a higher proportion of padding tokens for alignment requirements.} \Lan{Be consistent with "tasks" or "jobs"} 

In the {\em BatchFusion} process, when training data lengths vary, alignment is necessary and achieved by \textit{padding} tokens to match the length of the longest data in the iteration. Figure \ref{fig:pad} illustrates an example of a fused batch, with padding tokens occupying a significant proportion, resulting in lower overall throughput efficiency. Although these padding tokens do not directly impact model performance,
%or the training process,  
their inclusion results in computational inefficiency. A key objective of ASPEN is to improve effective throughput by devising efficient padding strategies, thereby mitigating the computational inefficiencies arising from variable data lengths. 
%However, variable training data lengths require alignment through {\em padding tokens}, which, despite not affecting training quality,\Lan{pls use less interjections} consume considerable computational resources and decrease training throughput.
%First, by combining, or fusing, training data from various fine-tuning jobs into a single batch, ASPEN allows multiple LoRA modules to concurrently share the same pre-trained model during training. However, when training data lengths vary, alignment is needed and achieved by adding padding tokens to match the length of the longest data point. While these padding tokens do not have any impact on the model training, they consume significant computational resources, reducing {\em effective} training throughput. For example, in Figure~\ref{fig:pad}, the white part indicates non-effective throughput, while the colored part represents effective throughput. One of the key objectives in ASPEN is to increase the effective throughput by developing efficient padding strategies to mitigate the impact of variable data lengths on overall computational efficiency.
%First, when fusing batches from multiple LoRA fine-tuning jobs, special tokens, e.g. padding tokens, are required for dimension alignment during matrix calculations due to varying lengths of training data across different jobs. These special tokens do not have any impact on the model training but will consume computational resources, consequently reducing effective throughput. As depicted in Figure \ref{fig:pad}, padding issues are encountered. These blocks represent tokens trained in a unit of time, therefore the white part indicates non-effective throughput, while the other colored part represents effective throughput. Therefore, a key objective during the model fine-tuning process is to increase the effective throughput. This could involve developing more efficient padding strategies to minimize the impact of variable sequence lengths on overall computational efficiency.
%Secondly, If the weights of a pre-trained model can be shared during parallel multi-job training, and computing resources are allocated reasonably during the training process, it is possible to maximize the utilization of computing resources in the fine-tuning process of multi-jobs. This can enhance the overall throughput of the system and reduce end-to-end latency in multi-job training.
% this is not clear:  early stop issues in the model fine-tune 
% $J_1, J_2, J_3, J_4$ demonstrate varying loss ratios or accuracy during fine-tuning. 
% Moreover, there's a clear opportunity to develop a predictive model to understand these early stop trends. 
% Such a predictive model would need to dynamically analyze ongoing job performance metrics and make real-time decisions, ensuring that GPU resources are allocated to the most promising jobs at any given moment. 
% Implementing this approach can significantly streamline GPU utilization, especially in environments where multiple fine-tuning jobs are run simultaneously.

%Training multiple fine-tuning jobs on a single GPU -- with constrained resources -- further requires maximizing resource usage and hence increasing overall system throughput. \Lan{} 
Training multiple LoRA fine-tuning jobs on a single GPU with limited resources requires significant resource management.
As depicted in Figure \ref{fig:early-stop} (left side), based on the loss or accuracy trends, $J_2$ and $J_3$ should be terminated early, as continuing to run those jobs with minimal gains consumes valuable compute resources without notable benefits.
%Secondly, when scheduling multiple fine-tuning jobs on a single GPU, it is crucial to consider scenarios where early stopping is applicable, and its trends are predictable. These factors significantly influence the overall fine-tuning scheduling strategy. For instance, as depicted in the left side of Figure \ref{fig:early-stop}, the loss or accuracy trends indicate that, for example, $J_2, J_3$ could be terminated early at a specific time point. Without early stop considerations, continuing to run those jobs with minimal improvements consumes valuable compute resources without significant benefits. 
Moreover, maximizing resource usage also needs to limit training errors. For example, concurrently running too many jobs can maximize resource usage but risks out-of-memory errors. Dynamic allocation of resources, such as GPU memory, to each job is critical, yet predicting the exact memory needs during scheduling is challenging.
ASPEN overcomes these challenges by developing delicate models to 1) predict when a job is unlikely to make further progress for early termination and 2) estimate the memory requirements of running jobs, avoiding out-of-memory errors. 
%These strategies enhance computational resource efficiency and reduce the overall job completion time.
%while optimizing for resource usage.
%ASPEN addresses this by predicting when a job is unlikely to make significant further progress, allowing for early termination. This strategy enhances computational efficiency and reduces the overall job completion time.

%Thirdly, in the fine-tuning process of LoRA models, the pre-trained model weights were frozen, resulting in multiple read-only pre-trained model weights reserved in memory during the training of multiple jobs. This redundant pre-trained weight data led to memory wastage. Secondly, accurately determining the computational resource requirements for each job at a specific time point and performing effective computational resource allocation at the job level proved to be highly challenging during the training process.
% this is not clear: dynamic number of jobs fine-tuning in parallel and oom issues

%Last, when scheduling multiple fine-tuning jobs on a single GPU, it is vital to dynamically allocate appropriate resources (e.g., GPU memory) to each job. GPUs can typically handle multiple jobs simultaneously, and the memory size of each job is uncertain during each scheduling. 
%If there are too many jobs running concurrently, it may lead to out-of-memory issues, and vice versa. %Conversely, if there are too few jobs, it may result in insufficient computational and memory usage. 
%Therefore, there is a clear need to develop a multi-LoRA fine-tuning memory usage model that accurately estimates the memory requirements of concurrently running jobs, optimizing for both throughput and memory utilization.

%Motivated by these considerations, we propose the Multi-LoRA Trainer, which involves sharing the weights of pre-trained model and performing resource allocation at the iteration level during the training process. However, implementing these ideas is not a trivial work and comes with the following challenges:
%\begin{itemize}
%    \item Fuse batch data from multiple jobs into a single batch to share pre-trained model weights poses challenges due to uneven length distributions in training data. Matrix operations require consistent dimensions, leading to the use of special tokens for padding to align the data. The special tokens used for padding can waste computational resources, thereby reducing throughput and increasing training latency;
%    \item Determining the optimal number of concurrently running tasks during the fine-tuning of multiple jobs can be challenging. If set too low, computational resources may not be efficiently utilized; if set too high, there is a risk of triggering Out of Memory (OOM) errors. Striking the right balance requires careful consideration of the available resources and the complexity of the fine-tuning tasks to ensure efficient utilization without compromising stability;
%    \item In scenarios involving hyperparameter searches and concurrent training of numerous models, the timely termination of underperforming tasks is crucial to prevent significant resource wastage. Implementing effective mechanisms for early stopping or automated evaluation of model performance can help mitigate this issue. It not only conserves computational resources but also streamlines the overall optimization process by allocating resources more efficiently towards promising configurations.
%\end{itemize}


To evaluate ASPEN, we fine-tuned several LLMs, including LLaMA-7B/13B~\cite{touvron2023llama1}, ChatGLM2-6B~\cite{du2022glm}, and LLaMA2-7B/13B\cite{touvron2023llama}. The results from these experiments highlight the efficiency of ASPEN in optimizing GPU utilization, GPU memory usage, and training throughput on a single GPU setup. When compared to Huggingface's PEFT~\cite{peft}, a leading parameter-efficient fine-tuning library employed by Alpaca-LoRA~\cite{alpaca-lora}, QLoRA~\cite{dettmers2023qlora}, and others, ASPEN showed a remarkable increase in throughput, achieving improvements of up to 17\%. These findings underscore the potential of ASPEN as a robust tool for enhancing the efficiency and performance of LLMs in resource-constrained environments.

In summary, this paper has the following contributions:

\begin{enumerate}
    \item We introduce the Multi-LoRA Trainer, enabling the efficient sharing of pre-trained model weights by {\em BatchFusion} method during the fine-tuning process of LLMs;
    \item We propose the Adaptive Job Scheduler, which collects various metrics from jobs and enables the accurate estimation of both the performance of the model and resource utilization, maximizing the system efficiency;
    %\item Upon the above two schemes, we implement ASPEN, a high-throughput large language model fine-tuning framework for training multiple LoRA modules in parallel.  \Lan{not a good contribution}
    %based on LoRA;
    \item ASPEN effectively uses computing resources, thereby improving training throughput and reducing training latency compared to state-of-the-art LoRA training systems. ASPEN saves 53\% of GPU memory when training multiple LLaMA-7B models on NVIDIA A100 80GB GPU and boosts training throughput by about 17\% compared to existing methods when training with various pre-trained models on different GPUs.
\end{enumerate}
%\vspace{-2em}



==> OLDVER/OLDVER/chapters/II._Background.tex <==

%In this section, we highlight the importance of fine-tuning LLMs and discuss the opportunities and challenges in parameter-efficient fine-tuning methods.

%\subsection{Fine-Tuning Pre-trained Models}

%Fine-tuning pre-trained models democratizes the benefits of large language models. 
%Training a large language model (LLM) from scratch requires a tremendous amount of time (e.g., several days on thousands of GPUs \cite{narayanan2021efficient}) and significant financial investment \cite{sharir2020cost}. For instance, training GPT-3 with 175 billion parameters necessitates 355 GPU-years, costing over 4 million dollars \cite{li2020openai}. Such high costs make it only affordable for a small proportion of individuals in the AI community.
\noindent\textbf{Fine-tuning pre-trained models.}
Training a large language model (LLM) from scratch requires substantial resources, both in terms of time and finances. It can take several days using thousands of GPUs~\cite{narayanan2021efficient} and entail significant financial investment~\cite{sharir2020cost}. 
Fine-tuning pre-trained models has democratized the access of the advantages of LLMs: Many organizations make their pre-trained models publicly available, such as Meta’s LLaMA \cite{touvron2023llama} and THUDM's GLM \cite{du2022glm}. These pre-trained models can be fine-tuned for various downstream jobs -- a method that has been proven effective~\cite{huang2020swapadvisor}. 
Thus, leveraging these publicly accessible pre-trained models via fine-tuning becomes the most feasible way to harness the benefits of LLMs.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{pics/ASPEN lora.pdf}
    \caption{Sharing pre-trained model weights for training multiple LoRA jobs with reduced overhead.}
    \label{fig:multi-lora}
    %\vspace{-1em}
\end{figure}

%\subsection{Parameter-Efficient Fine-Tuning Methods}
\label{sec:ftmethods}
\noindent\textbf{Parameter-efficient fine-Tuning methods.}
A {\em full-weight} fine-tuning of large-scale pre-trained models typically needs to update all parameters of the models and is often associated with prohibitive computational costs \cite{lv2023parameter}. 
In contrast, parameter-efficient fine-tuning (PEFT)~\cite{peft} methods 
%offer an effective means for adapting pre-trained models to diverse downstream applications without the need to fine-tune all model parameters. 
%The PEFT methods 
selectively fine-tune a few additional model parameters, resulting in substantial reductions in computational and memory resources. 
%Recent advancements in PEFT have demonstrated performance comparable to that achieved through full-weight fine-tuning.
% more citations here
As one of the state-of-the-art PEFT techniques, %LoRA~\cite{\cite{hu2021lora}} frees the weights of a pre-trained model and the preservation of model update weights through an Adapter, thereby significantly reducing graphics memory requirements during training while maintaining model accuracy. For instance, in the case of GPT-3 175B, it reduces the required graphics memory for training from 1.2TB to 350GB.
%LoRA stands out as particularly noteworthy. Introduced in 2021 by Hu et al. \cite{hu2021lora}, 
%LoRA is primarily employed for fine-tuning jobs in large language models. The core principle of 
%LoRA involves the freezing of the weights of a pre-trained model and the preservation of model update weights through an Adapter, thereby significantly reducing graphics memory requirements during training while maintaining model accuracy. For instance, in the case of GPT-3 175B, it reduces the required graphics memory for training from 1.2TB to 350GB.
LoRA~\cite{hu2021lora} achieves efficient fine-tuning 
%with reduced resource requirements 
by completely freezing the pre-trained model and introducing weight modifications through a trainable low-rank decomposition matrix, as illustrated in Figure \ref{fig:multi-lora}(a) and expressed in Equation \ref{eq:lora}:
\begin{equation}
\label{eq:lora}
h = W_0x + \Delta Wx = W_0x + BAx
\end{equation}

where $x$ denotes the input batch of the fine-tune job, $W_0 \in \mathbb{R}^{d \times k}$ represents the frozen pre-trained model weights, and $B \in \mathbb{R}^{d \times r}$ and $A \in \mathbb{R}^{r \times k}$ are low-rank decomposition matrices, with the rank $r \ll \text{min}(d,k)$.

%In principle, LoRA can be applied to any subset of weight matrices in neural networks to reduce the number of trainable parameters. For simplicity and enhanced parameter efficiency, LoRA typically focuses on adjusting attention weights used in downstream jobs while keeping the multi-layer perceptron (MLP) module frozen.
% what are the attention weights

%\smallskip
\noindent\textbf{Opportunities: sharing pre-trained models.}
%In the LoRA approach, as depicted in Figure \ref{fig:multi-lora}(a), the weights of the pre-trained model are frozen, and sharing it during fine-tuning can be achieved by switching low-rank decomposition matrices $A$ and $B$ when transitioning between different jobs. Sharing pre-trained model weights can lead to substantial GPU memory savings when sequentially training multiple jobs using the same pre-trained model on a single GPU. PEFT has successfully facilitated this approach. According to the Formula \eqref{eq:lora}, this method is represented by multiplying several small matrices with a large matrix individually in the GPU computation process. However, performing a large number of operations that require small computational resources on the GPU can be inefficient, while executing a small number of operations that demand significant computational resources on the GPU can be more effective. We can find a way to save computational resources by aggregating these operations into a single operation.
%\Ye{As shown in Figure \ref{fig:multi-lora}(a), when fine-tuning multiple jobs using the LoRA method, due to weight freezing, these jobs can be executed sequentially. The low-rank matrices A and B are switched based on the currently executed job to achieve the purpose of sharing pre-trained weights. PEFT has successfully facilitated this approach. When each job is switched, the GPU consumes some time to launch all matrix multiplication and addition operations in Equation \ref{eq:lora}. Since the pre-trained matrix $W_0$ does not change, it means we can merge multiple input training data $x$ into a larger matrix for matrix multiplication, reducing the number of times matrix multiplication needs to be launch.}
Figure \ref{fig:multi-lora}(a) illustrates a typical way to train a single LoRA fine-tuning job from a pre-trained model. When training multiple LoRA fine-tuning jobs {\em using the same pre-trained model}, sharing pre-trained models among all jobs seems intuitive to save GPU memory.  A straightforward way to achieve this is by {\em only} swapping the low-rank matrices A and B for each job while keeping the pre-trained model in GPU memory. This way, multiple jobs are trained separately and sequentially meanwhile sharing the same pre-trained model. 
%Indeed, existing approaches like PEFT have adopted this approach.
According to Equation \ref{eq:lora}, the matrix $x$ formed by the training data of each job is multiplied individually with the shared pre-trained model weights during the fine-tuning process of multiple LoRA jobs.
Despite being simple, training multiple LoRA jobs sequentially may not be the most efficient approach in terms of resource utilization and training performance. 

We have noted that the kernel launch cost incurred with each matrix multiplication and addition operation plays a substantial role in the overall training execution time.
%(e.g., 50\% of GPU time). 
%We observe that the kernel launch cost associated with every matrix multiplication and addition operation contributes significantly to the overall training execution time. 
%and these costs are not influenced by the complexity of these operations or the size of the matrix~\cite{zhang2019understanding}. 
Further, we observed that if we can train multiple LoRA jobs in parallel, as shown in Figure \ref{fig:multi-lora}(b), by ``merging'' individual jobs' training data into a large matrix before multiplying it with the shared pre-trained model weights, the number of matrix multiplications can be reduced significantly (i.e., reduced launch costs), compared with the sequential training approach. Inspired by these observations, we propose a novel BatchFusion technique at \S\ref{sec:BatchFusion}.
%This method enables more efficient sharing of a pre-trained model during the training of multiple LoRA fine-tuning jobs, as detailed before. 

%\smallskip
\noindent\textbf{Challenges: maximizing resource utilization.}
%In existing single-job training systems, such as Alpaca-LoRA based on PEFT, efficient utilization of system resources poses a challenge. This challenge stems from the difficulty in maximizing resource utilization for individual jobs, as the length of training data dynamically varies during the training process, resulting in fluctuating GPU memory occupation. Therefore, it is crucial to estimate hyperparameters based on the maximum GPU memory usage before training begins. The attempt to achieve multi-job training through parallel execution of multiple single-job training systems exacerbates resource wastage: each job stores a copy of pre-trained model weights in GPU memory, and these jobs compete for GPU computational resources without a strategic allocation approach.
%\Ye{In scenarios with limited memory resources, it is often impossible to run all jobs simultaneously. How to schedule the running order of jobs to maximize the utilization of computational resources and improve system performance becomes a challenge. Unlike job scheduling algorithms in operating systems, in the scenario of using LoRA fine-tuning with multiple jobs, the memory usage of each job can be estimated in advance, and the early stopping prediction model makes the runtime of jobs predictable. This requires a scheduling algorithm that is more suitable for scheduling LoRA fine-tuned jobs.}
While training multiple LoRA jobs can more efficiently use computational resources and reduce training overhead,
in scenarios with limited memory resources, running all jobs simultaneously is often impossible. The challenge then becomes how to schedule the running order of jobs to maximize the utilization of computational resources and improve system performance. Unlike other job scheduling algorithms (e.g., in operating systems), in the scenario of LoRA-based fine-tuning with multiple jobs, the memory usage of each job can be estimated in advance. Further, the early stopping prediction model makes the runtime of jobs predictable. This necessitates a scheduling algorithm that is more fitting for managing the scheduling of LoRA fine-tuning jobs.
%\vspace{-2em}

==> OLDVER/OLDVER/chapters/III._Overview.tex <==

In this section, we present an overview of the ASPEN architecture and highlight its key design objectives.

\smallskip
\noindent \textbf{Design objectives:}
ASPEN focuses on efficiently fine-tuning multiple LoRA jobs on a single GPU while effectively sharing pre-trained weights for these jobs. It dynamically schedules computational and memory resources for multiple LoRA jobs to optimize training throughput and resource utilization while maintaining model performance. The objectives of ASPEN are to answer the following two key questions:
\begin{itemize}
    \item \textit{How can pre-trained weights be effectively shared with minimal overhead to enhance training throughput?} (\S\ref{section:multi-lora-trainer})
    \item \textit{How can we adaptively schedule jobs by estimating various metrics of training jobs to meet diverse requirements?} (\S\ref{section:job-scheduler})
\end{itemize}

%\smallskip
\noindent\textbf{Architecture Overview:}
As illustrated in Figure \ref{fig:architecture}, ASPEN consists of three main components:
\begin{itemize}
    \item A self-supervised language model trainer that can handle multiple LoRA fine-tuning jobs, called the \textit{Multi-LoRA Trainer} (\ding{186});
    \item A profiler collecting various metrics of running jobs and producing estimated results for these metrics (\ding{184});
    \item A job scheduler that can chooses a scheduling strategy based on the estimated results from the profiler and user requirements (\ding{185}).
\end{itemize}

%\smallskip
\noindent\textbf{ASPEN's fine-tuning workflow:}
As depicted in Figure \ref{fig:architecture}, users initiate requests to ASPEN (\ding{182}), providing hyperparameter configurations, training data, and scheduling objectives, which include minimizing waiting time, reducing turnaround time, maximizing throughput, among others, as elaborated in \S\ref{section:job-scheduler}. Subsequently, ASPEN generates multiple candidate jobs (\ding{183}) based on this information and configures estimated fundamental parameters for each job in the Profiler (\ding{184}) during system initialization.

Once the system is initialized, the Scheduler (\ding{185}) selects a subset of jobs from the candidates, aligning them with user-defined scheduling objectives, and submits them to the Multi-LoRA Trainer (\ding{186}) for concurrent training. The Multi-LoRA Trainer (\ding{186}) provides performance metrics for the training jobs to the Profiler (\ding{184}) for estimation. The iteration of these steps (\ding{184}\ding{185}\ding{186}) constitutes one training cycle, repeated until all candidate jobs (\ding{183}) have completed their training.

In the event of new requests (\ding{182}) during training, ASPEN asynchronously generates candidate jobs (\ding{183}) based on the information provided in the requests. Subsequently, in the Profiler (\ding{184}), estimated fundamental parameters are configured for each job. The candidate job set is then updated before the commencement of the next iteration, ensuring that the training process incorporates the latest input seamlessly.
%\vspace{-1em}

==> OLDVER/OLDVER/chapters/IV.___V._Method.tex <==
\section{Multi-LoRA Trainer}\label{section:multi-lora-trainer}

In this section, we present the details of the \textit{Multi-LoRA Trainer}, focusing on how it can efficiently share pre-trained weights across parallel LoRA fine-tuning jobs using a novel technique called {\em BatchFusion}. We then examine the costs associated with this approach. Further, we address a critical challenge encountered during the {\em BatchFusion} process, i.e., the issue of padding. To mitigate this, we introduce the \textit{OptimalBatch} algorithm, aiming to minimize the impact of padding and optimize the overall fine-tuning process.
%\vspace{-0.5em}
\subsection{Batch Fusion}\label{sec:BatchFusion}
%Efficient Sharing of Pre-trained Weights}

%Sharing pre-trained weights is not a novel concept. In fact, due to the relatively small size of each LoRA module, typically it is only a few tens of megabytes to a few hundred megabytes in size, simultaneously storing several LoRA modules in the graphics memory is not challenging. 

%As shown in Figure~\ref{fig:multi-lora}(a), the LoRA implementation~\cite{peft} allows {\em one} LoRA module to engage in computation during each training iteration. This requires the (costly) switching of low-rank decomposition matrices $A$ and $B$ when transitioning between different fine-tuning jobs. 
%Figure \ref{fig:multi-lora}(a) illustrates an example of a LoRA fine-tuning job. When performing multiple LoRA fine-tuning jobs with the same pre-trained model, the model can be shared by switching the low-rank matrices A and B for each job and executing the jobs one by one.
%Mingjie to Ye: Exaplain the drawback for the previous work
%Show some number to demonstrate it is costly
Unlike the existing model-sharing approach in training multiple LoRA fine-tuning jobs (stated in \S\ref{sec:ftmethods}), we propose a novel {\em BatchFusion} technique for more efficient sharing a pre-trained model when training multiple LoRA fine-tuning jobs, as illustrated in Figure~\ref{fig:multi-lora}(b). {\em BatchFusion} fuses training data from {\em multiple} fine-tuning jobs into one batch before each training iteration; thus, multiple LoRA modules can share the same pre-trained model and participate in training {\em in parallel} in every iteration (instead of training sequentially or individually). The benefits of the proposed shared infrastructure are twofold: 1) It parallelizes the fine-tuning process by avoiding frequent swappings between fine-tuning jobs and mitigating model switching overhead. 2) It further optimizes the use of GPU resources by reducing kernel launch costs, thereby enhancing overall computational efficiency.

Specifically, the \textit{Multi-LoRA Trainer}
facilitates the parallel execution of multiple fine-tuning jobs on the same GPU. In Figure~\ref{fig:multi-lora}(b), consider multiple LoRA fine-tuning jobs, $J_1, ..., J_n$. Each job $J_i$ involves fine-tuning input data denoted as $x_i$. The low-rank decomposition matrices for the i-th job ($J_i$) are labeled as $A_i$ and $B_i$. Notably, all these jobs share the same pre-trained weights, represented by $W_0$. 
Formally, let $Fusion$ represent the {\em BatchFusion} process, and $Concat$ represent the matrices concatenation operation; the $Fusion$ operation is similar to matrix concatenation, but we add additional padding tokens to ensure {\em dimension alignment}, along with extra information to identify which LoRA module the input data belongs to. Thus, given the input batch for the i-th job $x_i$, the output data will be $h_i$. The fused batch matrix is $X=Fusion(x_{1},\dots,x_{n})$. It will be multiplied with the pre-trained weights and all LoRA module weights, and the individual results are then added together to produce the final output $H$. The complete calculation formula is shown as follows:
\begin{align}
    \label{eq:multi-lora}
     H &= Concat(h_{1},\dots,h_{n}) 
       = W_0X + [\Delta W_1x_{1},\cdots,\Delta W_nx_{n}] \nonumber \\
       &= W_0X + [B_1A_1x_1,\cdots,B_nA_nx_n]
\end{align}

where $W_0 \in \mathbb{R}^{d \times k}$ denotes the shared pre-trained weights; $\Delta W_i = B_iA_i$ denotes the weights of the LoRA module trained by the i-th job, where $B_i \in \mathbb{R}^{d \times r_i}$ and $A_i \in \mathbb{R}^{r_i \times k}$ are low-rank decomposition matrices, with the rank $r_i \ll \text{min}(d,k)$.

%\subsection{Cost Analysis for Multi-LoRA Batch Fusion}
%\vspace{-0.5em}
\subsection{Cost Analysis}
\label{sec:costanalysis}
%In this section, we analyze the GPU memory usage for the batch fusion approach. 
To understand how the fusion of training data points from multiple fine-tuning jobs impacts the overall resource usage of the GPU, we analyze and evaluate the GPU memory usage and computation cost associated with the {\em BatchFusion} approach.

%\smallskip
\noindent\textbf{Memory cost.}
We observed that no popular system currently facilitates the sharing of pre-trained models for training multiple fine-tuning workloads. Therefore, we compare the GPU memory usage between the {\em BatchFusion} approach and the commonly used single-job LoRA fine-tuning system, i.e., Alpaca-LoRA~\cite{alpaca-lora}.
We assume 1) the weight of each individual LoRA model denoted as \( W_l \), 2) the weight of the pre-trained base model represented as \( W_p \), and 3) the additional memory required for training each LoRA model denoted as \( W_e \). %we can quantify the memory efficiency gained through Batch Fusion in a multi-job scenario. Specifically, 
When running \( k \) concurrent fine-tuning jobs on the same GPU, the total GPU memory required by the Alpaca-LoRA system (without {\em BatchFusion}) is $k(W_p+W_l+W_e)$ -- though running in parallel, each training job has its own copy of the pre-trained weight.
In contrast, the {\em BatchFusion} approach reduces the need to replicate the pre-trained model weight \( W_p \) for each job. Therefore, with \( k \) jobs, {\em BatchFusion} saves \( (k-1)W_p \) GB in GPU memory, thereby enhancing memory efficiency. 
%Using Multi-LoRA Trainer, we can share the pre-trained model with a memory size of $W_p$, resulting in a GPU memory usage of $W_p+k(W_l+W_e)$.
%By training multiple fine-tuning jobs in parallel, the Batch Fusion approach allows these jobs to share the same shared pre-trained model, thereby enhancing memory efficiency. 
As a concrete example, using quantized (e.g., 8-bit) LLaMA-7B models, {\em BatchFusion}  can save the total memory amounting to \(7(k-1)\) GB. 
%This batch fusion approach capitalizes on the shared pre-trained model weights across different fine-tuning jobs, thereby enhancing memory efficiency. It achieves this by eliminating the need to store multiple instances of the same base model weight for each fine-tuning job. Consider, for example, the use of quantized (i.e., 8-bit) LLaMA-7B models. In such a scenario, the total memory savings can amount to \(7(k-1)\) GB, which is a considerable reduction. 
%We have validated this theoretical conclusion with practical experiments, as depicted in Figure \ref{fig:exp-mem}.
%Mingjie: do we need to refer this ?
%In these experiments, employing a batch size of 6, the traditional approach without Multi-LoRA Trainer consumes 33GB of memory when training three LoRA models. In contrast, by utilizing the Multi-LoRA Trainer, we observed a memory usage reduction of 14GB. This efficient use of memory allows for training up to an additional 6 times more LoRA models concurrently, showcasing the significant benefits of this method in terms of memory savings and increased training capacity on a single GPU.

% Mingjie to Ye: what is the meaning for this part

%\begin{lemma}\label{lemma:kernel-launch-with-same-time}

%\end{lemma}

%\begin{figure}
%    \centering
%    \includegraphics[width=0.8\linewidth]{pics/Overheads of CUDA Kernels.pdf}
%    \caption{The overheads of launching CUDA kernels.}
%    \label{fig:kernel-overheads}
%    \vspace{-13pt}
%\end{figure}

%\smallskip
\noindent\textbf{Computation cost.}
%In the GPU computing process, each computational operation needs the launching of a kernel. However, the overhead associated with the kernel launching can be nontrivial~\cite{zhang2019understanding}.
%\Ye{In the GPU computing process, before each computational operation e.g.Matrix multiplication and addition, needs takes some time to launch the kernel. However, the overhead associated with the kernel launching can be nontrivial~\cite{zhang2019understanding}.}
In GPU computation, before each operation, there is a need to launch the kernel to execute matrix multiplication and addition, and the overhead associated with this kernel launching can be nontrivial. This overhead is particularly impactful in the case of small kernels, i.e., kernels with computations for lower rank matrices~\cite{zhang2019understanding}. This observation leads us to:

% Launch a new kernel when the performance improvement surpasses the overhead of a new kernel.

% fixing the reference inconsistency
%Zhang et al. (2019) employed the micro-benchmark method to assess various overheads during the kernel execution process, emphasizing that the overhead of the kernel launch cannot be overlooked \cite{zhang2019understanding}. 
%For example, 
%Figure \ref{fig:kernel-overheads} illustrates the overheads of launching CUDA kernels with two sizes, representing a small kernel and a large kernel separately. The left part represents the overhead for the execution of a small kernel with no code inside, and the right part represents the overhead for the execution of a large kernel containing code sleeping for 1000 ns. The \textit{Batch Fusion} approach of the Multi-LoRA Trainer assembles the right part, i.e., a larger kernel instead of multiple small kernels. We can observe from the figure that the execution latency and additional latency change together with the size of the kernel, while the kernel launch latency remains nearly the same (and contributes to a very significant portion of the overall execution time). Hence, we have the lemma as follows:
%\Ye{Figure \ref{fig:kernel-overheads} illustrates the overheads of launching CUDA kernels with two sizes, representing a small kernel and a large kernel separately. The left part represents the overhead for the execution of a small kernel with multiplication of smaller matrices(e.g. in the Equation \ref{eq:lora} $Wx$), and the right part represents the overhead for the execution of a large kernel with multiplication of larger matrices(e.g. in the Equation \ref{eq:multi-lora},$WX$, the matrix $X$ bigger than $x$ ). The \textit{Batch Fusion} approach of the Multi-LoRA Trainer assembles the right part, i.e., a larger kernel instead of multiple small kernels. We can observe from the figure that the execution latency and additional latency change together with the size of the kernel, while the kernel launch latency remains nearly the same (and contributes to a very significant portion of the overall execution time). Hence, we have the lemma as follows:}

%Figure \ref{fig:kernel-overheads} illustrates the overheads of launching CUDA kernels with two sizes, representing a small kernel and a large kernel separately. The left part represents the overhead for the execution of a small kernel with the multiplication of smaller matrices (e.g., similar to $Wx$ in Equation \ref{eq:lora}), and the right part represents the overhead for the execution of a large kernel with the multiplication of larger matrices (e.g., similar to $WX$ in Equation \ref{eq:multi-lora}, where $X$ is composed of multiple matrices $x$). 
%Note that the with {\em BatchFusion} approach corresponds to the right part of the figure, i.e., using a larger kernel instead of multiple small kernels. 

%We observe that while the GPU execution latency and additional latency (data transfer, synchronization, etc.) increase as the kernel size increases, the kernel launch latency almost remains the same; additionally, the kernel launch contributes to a significant portion of the overall execution time. This observation leads us to:

%training multiple fine-tuning jobs in parallel can reduce the computation costs associated with the kernel launching. 
%Thus, we can reduce computation costs during the forward process by minimizing kernel launches.
% from this figure, left is sth, right is sth, in this figure, blue, red, dark 
% in this application, we focus the sitaution as the right part. 
% we can observe that sth...
% thus, we can do sth, luanch kernel cost is constant different cases, thus we do sth. 

%\begin{lemma}

%\end{lemma}
%\Tang{can save space here}
Fusing multiple small kernels into a large kernel can reduce overall computation costs by saving kernel launch costs; it can effectively reduce approximately 30\% - 50\% of the theoretical kernel launch costs. For example, given that PEFT \cite{peft} is a widely used fine-tuning library employed by Alpaca-LoRA~\cite{alpaca-lora}, QLoRA~\cite{dettmers2023qlora}, and others, we analyze the computation cost for the Multi-LoRA Trainer and PEFT as below. 

Assume there are $k$ LoRA fine-tuning jobs, each with a different training dataset. The input batch in each iteration can be denoted as $x_1,\cdots,x_k$, and the fused batch $X=Fusion(x_1,\cdots,x_k)$. When running these $k$ LoRA fine-tuning jobs on a single GPU, the computation cost mainly includes \textit{kernel execution cost} and \textit{kernel launch cost}.

%\smallskip
\noindent\textbf{Kernel execution cost.}
According to Formulas (\ref{eq:lora},~\ref{eq:multi-lora}), the primary kernel execution cost involves matrix multiplication and addition operations. Because ASPEN does not introduce additional calculations, it shall have the same computational complexity as PEFT. Therefore, we consider the kernel execution cost of {\em BatchFusion} in ASPEN and the existing PEFT method to be the same.

%\smallskip
\noindent\textbf{Kernel launch cost.}
Since the fused batch $X$ is composed of multiple input batches $x_i$, it follows that $r(x_i) < r(X)$. In computational operations involving matrix multiplication and addition, each operation initiates a kernel launch. As mentioned earlier, the overhead of kernel launches is particularly impactful for small kernels, i.e., kernels with computations for lower-rank matrices. Referring to Formulas (\ref{eq:lora},~\ref{eq:multi-lora}), the PEFT method requires $4k$ small kernel launches for $k$ fine-tuning jobs, each job involving three multiplications and one addition operation.

In contrast, the \textit{BatchFusion} approach reduces the number of small kernel launches to $2k$, each with one multiplication operation. Additionally, it introduces two large kernel launches composed of an addition and a multiplication operation. Since the overhead of kernel launches for large kernels, i.e., kernels with computations for higher-rank matrices, is similar to that for small kernels, we infer that the total time spent on kernel launches is directly proportional to the number of launches. Therefore, the proposed \textit{BatchFusion} approach effectively reduces the theoretical kernel launch costs by approximately $(2k-2)/4k$. 
% \Tang{In practice, where the number of jobs is typically three or more, this translates to a 30\% to 50\% reduction in kernel launch costs}. 
% This significant decrease in kernel launches enhances the efficiency of the GPU and results in faster computation times in the fine-tuning process.

%Formally, let \(\varphi\) represent the cost associated with each kernel launch, \(\zeta\) denote the overhead incurred by the \textit{Fusion} process in {\em BatchFusion}, and \(\delta\) represent the overhead for switching low-rank decomposition matrices in the PEFT approach (i.e., training multiple jobs sequentially). For PEFT, the total computational cost can be expressed as \( C + 4k\varphi + k\delta \), where \( C \) represents the base computational cost. On the other hand, for the {\em BatchFusion} method, the computation cost is given by \( C + (2k+2)\varphi + k\zeta \). Hence, the reduction in the total computation cost achieved by {\em BatchFusion}, as compared to PEFT, is \( 2\varphi(k-1) + k(\zeta - \delta) \). This indicates that while the {\em BatchFusion} approach does not reduce the actual GPU computational workload, it effectively cuts down the theoretical kernel launch costs by approximately 30\% to 50\%. %This reduction is primarily achieved by decreasing the number of kernel launches, thus optimizing the overall computational efficiency without compromising the workload processed by the GPU.


\noindent\textbf{Summary.}
%Therefore, we conducted an analysis of memory usage and computation cost for the Multi-LoRA Trainer of ASPEN. 
The {\em BatchFusion} approach devised in ASPEN can save $(k-1)W_p$ GB of GPU memory and approximately 30\% to 50\% of the kernel launch costs compared to the state-of-the-art PEFT method.

% \Tang{Therefore, we find that memory usage is sth, and the compuation cost is sth. This can improve the traditional approach by xxx.}

%Considering the additional overhead introduced by both methods, let $\delta$ be the module switch overhead for PEFT, $\zeta$ be the matrix concatenation overhead for Multi-LoRA Trainer, and $\varphi$ be the kernel launch overhead. The total computational cost $\Theta_m$ for Multi-LoRA Trainer and $\Theta_p$ for PEFT in the forward process can be denoted as:
%\begin{align}
%    \Theta_m &= (2k + 2)\varphi + \Theta(k) + k\zeta \\
%    \Theta_p &= 4k\varphi + \Theta(k) + k\delta
%\end{align}

%Since the module switch overhead $\delta$ and the matrix concatenation overhead $\zeta$ correspond to single matrix multiplication or addition operations in practice, the overhead is similar. For the sake of simplicity in analysis, we assume $\delta = \zeta$. Consequently, the saved computational cost by Multi-LoRA Trainer can be denoted as:
%\begin{equation}
%    \Delta\Theta = \Theta_p - \Theta_m = (2k - 2)\varphi
%\end{equation}

\subsection{Data Alignment and Padding}\label{sec:padding-issue}
%As mentioned in \S\ref{sec:BatchFusion}, the Batch Fusion method fuses training data from multiple fine-tuning jobs into a single batch before each training iteration. 
In the {\em BatchFusion} process, when training data lengths vary, alignment is needed and achieved by adding {\em padding tokens} to match the length of the longest data in the iteration. Although these padding tokens do not directly affect model performance or the training process, their inclusion leads to computational inefficiency. This is because these tokens increase the volume of data processed without contributing to actual training, thereby using computational resources without benefiting the training effectiveness.
%During the {\em BatchFusion} process, if the lengths of training data are different, it is necessary to align these data using special tokens with the longest training data of this iteration. While these special tokens do not impact model performance or the training process, they result in the inefficiency of computational resources.

% there are two training data in one iteration. It is evident that 
For instance, consider Figure~\ref{fig:pad}, which depicts four fine-tuning jobs, each with a batch size of 2, amounting to six training data points. These data points vary in length, with the longest being six units. To align data lengths, {\em padding tokens} are appended to the shorter data points. 
%This example illustrates that an increased proportion of padding tokens correlates with a decreased proportion of tokens actively involved in the training. 
Consequently, this leads to a less efficient use of computational resources.

%For example, in Figure \ref{fig:pad}, given four fine-tuning jobs, each configured with a batch size of 2, there are eight training data points. The lengths of these training data points vary, with the largest length of 8. To align these training data with the largest length, \textit{padding} tokens are added to the end of each training data point.
% \Tang{For this figure, job one have training token, we pad xxx the rest of trainig data. By this way, we can ensure taht xxx}
%From this example, we can tell that the higher the proportion of the padding tokens, the lower the proportion of tokens participating in the training, resulting in wasted computation resources. 

Formally, we introduce the concept of the \textit{padding ratio}, denoted as $\delta$, representing the proportion of the padding tokens in one batch. Let $\xi$ represent the total count of tokens in a fused batch, and $\xi_p$ represent the count of padding tokens in a fused batch. Then, $\delta$ is expressed as $\delta = \xi_p/\xi$.
%The Padding Ratio reflects the proportion of tokens in a single batch that do not participate in training. The lower this ratio, the greater the number of tokens actually involved in the training process. Importantly, it dynamically changes in real-time with training iterations.
%The Padding Ratio $ \delta$ reflects the additional computation rate during the model training process that does not affect the model's performance. The higher the ratio, the more computational resources are wasted. 
Notice that, for fine-tuning jobs sharing the same input training data, such as hyperparameter search scenarios, the training input data for each job is the same. Thus, we do not need to introduce padding tokens, and the $\delta$ is 0.
On the other hand, in scenarios involving fine-tuning jobs addressing distinct domain issues \cite{vicuna2023,jiao2023panda,xu2023baize,li2023chatdoctor,hu2023llmadapters}, each job would use diverse training datasets. These datasets may have different length distributions, and thus the length of training data in each iteration will vary, resulting in a higher $\delta$.
%and resulting in more padding tokens generated during the Batch Fusion. 
For exmaple, Figure~\ref{fig:data_distribution} shows the distribution of data lengths for different datasets, which can significantly differ from each other.

%Indeed, the length of training data is inherently randomly distributed, and the padding issue is present even in single-job training systems. However, when dealing with multiple jobs, Batch Fusion can exacerbate this problem.

%While $Padding Ratio$ effectively reflects the impact of additional padding tokens on the system, it may not be the most suitable metric for evaluating system performance. In the fine-tuning process of language models, we use throughput to represent the number of tokens the system can train per second.

We categorize the job throughput into two parts: the {\em effective throughput} and the {\em non-effective throughput}. Specifically, the non-effective throughput refers to the number of padding tokens computed by the system per second. The remaining part would be the effective throughput. Intuitively, a higher padding ratio would lead to worse effective throughput. Let $t$ represent the processing time, and $\sum token$ represent the total number of tokens processed in this period. $T_{tot}$ is the throughput, and the non-effective throughput $T_{non}$ and the effective throughput $T_e$ can be denoted as:
\begin{equation}
    T_e = T_{tot} - T_{non} = (1-\delta)T_{tot} = (1-\delta)\frac{\sum token}{t}
\end{equation}

Therefore, our goal is to reduce the padding ratio $\delta$ while improving the effective throughput $T_e$.

%$T_e$ eliminates the impact of padding tokens, effectively measuring the actual performance of the system. As the average value of $PaddingRation$ decreases, $T_e$ will increase accordingly. However, this raises a question: \textit{how can we increase effective throughput by reducing the padding ratio?}

%\subsection{Minimizing Padding Ratio}\label{section:fussion}
\smallskip
\noindent\textbf{Minimizing padding ratio.}
Drawing inspiration from Zhang et al.~\cite{zhang2021reducing}, we introduce the \textit{OptimalBatch} algorithm to minimize the padding ratio in training datasets. The \textit{optimal-batch} algorithm executes the following key steps in each iteration of the training process: First, it sorts each job according to the length of its training data. Next, it selects either the shortest or the longest training data from each job. Finally, it employs the {\em BatchFusion} operation (as detailed in \S\ref{sec:BatchFusion}) to combine these selected training data. This fused data is then fed into the Multi-LoRA Trainer for processing.

However, this approach faces two main challenges: 
1) Training models with sorted data can lead to issues with model performance convergence. As depicted in Figure \ref{fig:abnormal-loss}, one can observe two distinct loss curves. The abnormal curve on the left exhibits fluctuating behavior, failing to show a clear trend toward convergence, in contrast to the stable and converging curve on the right.
%Figure \ref{fig:abnormal-loss} shows an example of two loss curves. The abnormal loss curve on the left side fluctuates rather than showing a convergence trend, unlike the normal loss curve on the right side.
2) Implementing this method requires all jobs to be stored in GPU memory to determine the optimal batching solution. It becomes problematic in memory-constrained environments, particularly when managing a large number of jobs, as it can lead to out-of-memory errors. A potential approach is to select a subset of jobs fitting within memory limits. However, identifying the most suitable subset for optimal results is nontrivial.
%All jobs participating in the training need to be held in GPU memory to find an optimal batching solution. In memory-constrained environments with a large number of jobs, out-of-memory issues become critical. Selecting a subset of jobs that meets memory constraints can address this issue, but finding the optimal subset is not a trivial work.
%\Ye{Memory is limited, and if all jobs participate in training during each iteration, when there are many jobs, the fused training data after Batch Fusion will lead to out-of-memory issues. To address the issue, we can rearrange the execution order of jobs, but finding the optimal job execution order is not a trivial work.}
% b) Sorting can only aggregate data with similar distributions. When there is a significant disparity in the distributions of datasets used by different jobs, it becomes less effective. As illustrated in Figure \ref{fig:data_distribution} for LLaVA \cite{liu2023visual} dataset (marked with yellow color) and Spider dataset \cite{yu2019spider} (marked with blue color), the distributions of these two datasets are entirely different. In this scenario, the length of training data retrieved from these two jobs by \textit{OptimalBatch} will be significantly different, leading to a large number of padding tokens when applying the Batch Fusion operation.
Thus, we introduce the \textit{Job Scheduler} to address these challenges in Section~\S\ref{section:job-scheduler} .

%To address the issue, we can rearrange the execution order of jobs, but finding the optimal job execution order is not a trivial work.



\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{pics/Abnormal_loss.pdf}
    %\vspace{-20pt}
    \caption{An abnormal loss curve and a normal loss curve.}
    \label{fig:abnormal-loss}
    %\vspace{-10pt}
\end{figure}

\section{Job Scheduler}\label{section:job-scheduler}
In this section, 
%we discuss how to schedule jobs in such GPU memory-constrained environments. 
we first present a near-optimal approach to reduce the impact of padding tokens on training throughput. We then introduce an adaptive job scheduling algorithm incorporating early stopping predictions and memory usage estimation models.
%to improve system throughput and prevent out-of-memory.
%decrease job turnaround time, and reduce job waiting time.

%\subsection{Optimizing Training Throughput: A Scheduling Approach with the MinPad Algorithm}\label{section:minpad}
\subsection{Optimizing Training Throughput}\label{section:minpad}
%In scenarios like multi-user training, concurrently training dozens to hundreds of models is quite common. We have observed that when there's a good number of candidate jobs available, choosing jobs with similar data distributions for combined training can help lessen the effect of padding tokens on effective throughput.

%In accordance with Figure \ref{fig:minpad}, we have three jobs, and our memory only can hold two jobs, thus we can run two jobs at the same time.
%During the first iteration, employing the FIFO scheduling method for job selection will result in 4 additional padding tokens, but employing the MinPad algorithm only result in 1 additional padding token.

% This means we can only run two jobs simultaneously. 
Scheduling multiple jobs in a memory-constrained environment, such as a single GPU, is challenging. Figure \ref{fig:minpad} shows an example where only two jobs can fit. Though FIFO is a common scheduling approach~\cite{mohan2022looking}, it results in four padding tokens in the fused batch. In contrast, the $MinPad$ algorithm (our approach) reduces this to just one.

%\smallskip
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{pics/minpad.pdf}
    \caption{An example of the MinPad algorithm.}
    \label{fig:minpad}
    %\vspace{-2em + 5pt}
\end{figure}
\noindent\textbf{Observation:} when handling numerous candidate jobs, selecting jobs with similar data length distributions for the same batch can reduce the padding ratio, thus improving effective throughput.
%  a fine-tuning job consists of multiple iterations
%As mentioned earlier, in memory-constrained environments, we can only run a fixed number of jobs concurrently. Consequently, we need to schedule a specific number of diverse jobs for each iteration, necessitating the selection of a job set from the candidate pools in every iteration.

Based on this, we propose the $MinPad$ algorithm, to address the padding issues caused by {\em BatchFusion}: It first identifies the maximum number of jobs, $M$, that can be trained at the same time. Before each iteration, it reviews the data for each job and chooses $M$ training data with the fewest padding tokens.
%A detailed description of the algorithm can be found in Algorithm \ref{algo:minpad}.
$MinPad$ correlates the execution order with the distribution of training data lengths. While $MinPad$ ensures the minimum padding ratio, maximizing effective throughput, and avoids the unconvergence of each training process caused by sorting, it does not consider the priority, turnaround time, and waiting time of jobs. The priority scheduling algorithm is often used to manage job priority~\cite{zouaoui2019priority}, but this method does not consider the distribution of training data lengths, potentially increasing the padding ratio and reducing throughput, as discussed in \S\ref{sec:padding-issue}.
%\Tang{do we need to explain these points: potentially increasing the padding ratio and reducing throughput. give an example to explain this?} 


%\vspace{-0.5em}

\subsection{Early Stopping and Throughput Modeling}

% introduce the early stop and related motivation example

% introduce the resource usage modeling to reduce the issues xxx

%To address the drawbacks of the FIFO and priority scheduling strategies mentioned earlier and consider the characteristics of training large models: 1) During model training, early stopping may occur due to a decrease in accuracy or others. 2) Different input data sizes result in varying usage of memory resources. We propose an adaptive scheduling algorithm based on the predictable nature of these two characteristics. In this section, we provide a detailed description of enhancing system throughput by incorporating early stopping prediction. Subsequently, we utilize resource estimation to prevent out-of-memory issues and effectively leverage computational resources.
%In this section, we analyze how the early stop policy influences the job scheduling mechanism. 
In the model training process, if the model's performance deteriorates or remains unchanged, early stopping can be employed to terminate the training prematurely~\cite{dodge2020fine}. This approach avoids waiting to complete all training data, thus reducing unnecessary computation costs. As depicted in Figure \ref{fig:early-stop}, the lower-left corner displays the performance of four jobs during training. When calculating $J_2$'s loss value, a not-a-number ($NaN$) error occurs. If training persists, this error will recur, leading to abnormal model performance and wasted computing resources. $J_3$ and $J_4$ use various indicators to decide when to stop early. After each iteration, their accuracy is evaluated using a test set. $J_3$'s accuracy steadily declines during training, indicating that further training will not enhance performance and only waste resources. Therefore, it can be stopped early.


%\Tang{we need to explain the figure right part more clearly, and tell the reader what is the meaning of early stop, and how the early stop would influence the job schuedling. To simplify our discussion, we think each iteration share the constant run time cost.}

%In this study, we adopt the term iteration to denote varying steps, while ensuring that consistent runtime for each iteration.

%Each job comprises six iterations, and the system can simultaneously execute two jobs. Given the uniformity in priority and iteration numbers, a straightforward FIFO strategy can be employed for scheduling. In practice, the runtime of each iteration/step is different. 
%In this study, we adopt the term iteration to denote varying steps, while ensuring that consistent runtime for each iteration.

To simplify our discussion, we assume each iteration has a constant runtime, called iteration time. Four jobs, each with six iterations, were submitted concurrently. The system can run two jobs at once. Assuming equal priority for all four jobs, we compare three strategies: (a) a first-come, first-served scheduling strategy without early stopping; (b) a first-come, first-served strategy with early stopping; (c) a first-come, first-served strategy that includes both early stopping and a strategy that uses early stopping predictions for scheduling.

If we use strategy (a), six extra iterations will be done, wasting computational resources. Using strategy (b), the first step is to run $J_1$ and $J_2$ together. When $J_2$ encounters a $NaN$ error in its third iteration, it is stopped. Then, according to the first-come, first-served principle, $J_3$ starts running with $J_1$. After $J_1$ finishes, $J_4$ is scheduled to run alongside $J_3$.

Strategy (c) starts with a warm-up phase, where we run all jobs for two iteration times to gather prediction data. Then, scheduling is based on this data, prioritizing shorter jobs, $J_2$ and $J_3$, to increase throughput and reduce average turnaround time. In the given example, this method boosts throughput to 0.44 jobs per iteration time and lowers the average turnaround to 6.5 iterations per job. %Thus, including early stopping predictions in adaptive job scheduling is beneficial for enhancing system throughput.

%\smallskip
\noindent\textbf{Analysis between early stopping and throughout:}
To model the relationship between system throughput and early stopping, we consider a scenario where the total number of candidate jobs is $N$, and it is feasible to simultaneously run $k$ jobs. Each job involves $I_i$ iterations, and in the event of early stopping, the number of iteration times performed by each job is denoted as $L_i$, and the prediction accuracy is $\vartheta$. The set representing all training jobs is denoted as $\Gamma = \{L_1, L_2, \dots, L_N\}$. When utilizing prediction information for scheduling, the throughput is given by:
\begin{equation}
    T_{e} = \vartheta \frac{KN}{\sum_{i=1}^{N}L_i}
\end{equation}

The optimal throughput remains the same as $T_e$ without prediction information. However, in the worst-case scenario, the throughput may decrease to:
\begin{equation}
    T_{w} = \frac{N}{\sum_{i=1}^{k}\top_{k}\Gamma}
\end{equation}

Subsequently, we calculate its throughput as $T_{a} = (T_e+T_w)/2$. The throughput improvement using early stopping prediction information for job scheduling is determined by:
\begin{equation}
    \label{eq:early-stop-tp}
    \eta_{tp} = \frac{T_e-T_a}{T_a} = \frac{\tau - 1}{\tau + 1}\quad(\tau = \frac{\vartheta k\sum_{i=1}^{k}\top_{k}\Gamma}{\sum_{i=1}^{N}L_i})
\end{equation}

% the higher the value of $\tau$, the greater the improvement in throughput. In other words,
Equation \ref{eq:early-stop-tp} suggests that a larger difference in the actual number of iterations executed by each job results in a greater improvement in throughput. Thus, we can apply the early stopping prediction method, similar to estimating the risk at specific time points of gradient flow\cite{ali2019continuous}. This method can improve system throughput $\eta_{tp}$ and the higher the prediction accuracy $\vartheta$, the greater the throughput.

\subsection{Fine-Tuning with Memory Usage Modeling}

%\begin{lemma}
   %LoRA GPU memory usage modeling 
   %Adaptive job scheduling through GPU memory profiling enables effective resource utilization and prevents out of memory occurrences.
%\end{lemma}

%In the process of model training, opting for a larger fused batch size introduces the potential for out-of-memory issues. As a precaution, the fused batch size is typically chosen based on the maximum memory usage to mitigate these concerns. Consequently, the size of the fused batch or the number of parallel jobs in each step is maintained at a fixed, smaller value. It's important to note that employing a reduced number of parallel jobs may lead to an underutilization of computational resources.

In the model training process, as depicted in Figure \ref{fig:data_distribution}, there is an uneven distribution of data; varying input data lengths lead to different GPU memory requirements. The left column of Figure \ref{fig:batchsize_seqlen_mem} shows that we fixed each job's batch size to 24 and then adjusted the input data length to ascertain the maximum number of jobs that can run without encountering out-of-memory issues on a 48GB GPU.


%To prevent out-of-memory issues, we constrain the number of simultaneously running jobs to 2, as depicted in Figure \ref{fig:data_distribution}. Because the fused batch size is proprotial to the number jobs running at the same time, thus, the fused batch size is determined by the sum of the batch sizes. As illustrated in Figure \ref{fig:jobs_memory}, each job's batch size is set to 24. For a sequence length of 1024, only two jobs can run simultaneously. 
%\Tang{introduce distribution is changing greatly, Examining the data distribution reveals that the majority of data lengths hover around 100.}
%This implies that, for the most part, it is feasible to simultaneously run six jobs. Consequently, when the parallel job quantity is limited to 2, computational resources are often underutilized.

Therefore, suppose that we know the amount of resources utilized by jobs in each step, it becomes possible to dynamically adjust the number of jobs that can be concurrently run. Initially, to estimate the resources required for each step of a job, we follow the previous work in Vijay et al. \cite{korthikanti2023reducing} to infer the functional relationship between memory size and the size of input training data. Subsequently, we conduct online model fitting in the following manner: we define the input sequence length as $L_n$ and the input batch size as $B_t$. We can then employ the following model to capture this association:
 \begin{equation}
    \label{eq:memory-size}
    M = \beta_0 + \beta_1B_tL_n + \beta_2B_tL_n^2
\end{equation}

where $M$ represents the required memory, and $\beta_0$, $\beta_1$, and $\beta_2$ are non-negative coefficients. Throughout the model training process, we consistently gather data points $(B_t, L_n, M)$ and utilize a non-linear least squares solver to determine the optimal coefficients for fitting this model. An example of model fitting during the training of the LoRA model with LLaMA-7B is shown in Figure \ref{fig:batchsize_seqlen_mem} (right column).

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{pics/jobs_memory.pdf}
%     \caption{}
%     \label{fig:jobs_memory}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{pics/join_sequence_length.pdf}
    \caption{The maximum number of jobs that can run simultaneously with different input sequence lengths and online model fitting for training the LoRA model (with LLaMA-7B quantified in 8bit on NVIDIA RTX A6000 48GB) is determined by the coefficients $\beta_0=6.56$, $\beta_1=1.42\times 10^{-3}$, and $\beta_2=-8.76\times 10^{-8}$.}
    \label{fig:batchsize_seqlen_mem}
    %\vspace{-2em + 5pt}
\end{figure}

In ASPEN, we incorporate a warm-up phase before the actual training. This involves selecting data with various batch sizes and sequence lengths to fit Equation \ref{eq:memory-size}. At each step, we collect data points to enhance the accuracy of this model. With this estimated information, we can avoid out-of-memory issues by ensuring the following equation holds at each schedule:
\begin{equation}
    \label{eq:schedule-by-memory-size}
     CS_{job} = \{X \mid X \subseteq S_{job} \land \textstyle \sum_{x \in X}x.m \leq M_{mem}\}
\end{equation}

where $S_{job}$ denotes all available jobs for scheduling, $M_{mem}$ is the current maximum available memory, and $x.m$ signifies the estimated memory size derived from Equation \ref{eq:memory-size}. Equation \ref{eq:schedule-by-memory-size} guarantees that the system prevents out-of-memory issues during runtime.

On the other hand, for efficient utilization of computational resources, we choose a set $S_{c}$ of jobs for concurrent execution. This set should ensure that the total memory of selected jobs is as close to $M_{mem}$ as possible. In other words, it should satisfy the following equation:
%\vspace{-6.5pt}
\begin{equation}
    \label{eq:optim-schedule-by-memory-size}
     S_{c} \subseteq CS_{job} \land (\forall S^{'} \subseteq CS_{job}, \textstyle \sum_{x \in S_{c}}x.m \geq \textstyle \sum_{x \in S^{'}}x.m)
\end{equation}

%\begin{minipage}{\linewidth}
\begin{algorithm}[!ht]
    \caption{Adaptive Job Schedule}
    \label{algo:adaptive-job-schedule}
    \begin{algorithmic}[1]
        \Require Job queue: $Q_{job}$, Maximum available memory: $M_{mem}$, User-defined parameter: $top\_k$
        \Ensure Scheduling result: \textit{R}
        \State $Q_{job} \gets$ SortBy($Q_{job}$, priority, submitted\_time)
        \State $C_{job} \gets$ GetFront($Q_{job}$, $top\_k$)
        \State $C_{job} \gets$ MemEstimate($C_{job}$)
        \State $C_{job} \gets$ EarlyStoppingPredict()
        \State $C_{job} \gets$ SortBy($C_{job}$, the\_num\_of\_iterations)
        \Comment{SJF}
        \State $R \gets \emptyset $
        \For{$x \in C_{job}$ }
            \If{GetMem($x$) + GetTotalMem($R$) $\leq$ $M_{mem}$}
                \State $R \gets R \cup x$
            \EndIf
        \EndFor
    \end{algorithmic}
\end{algorithm}
%\end{minipage}

%\subsection{Adaptive Job Scheduling with Metrics Estimation}\label{section:adaptive-job-schedule}
\subsection{Adaptive Job Scheduling}\label{section:adaptive-job-schedule}

Based on early stopping prediction information and profile information on GPU memory, we propose an adaptive job scheduling to achieve: \ding{182} less waiting time, \ding{183} less turnaround time, \ding{184} large throughput, \ding{185} no out-of-memory issues, \ding{186} priority and fairness (high priority takes precedence, first come first serve). It is worth noting that the job scheduling problem is acknowledged as an NP problem \cite{ullman1975np}, and finding a solution that satisfies all the mentioned conditions is extremely challenging.

Taking inspiration from the operating system's completely fair scheduling algorithms \cite{kobus2009completely} and shortest job first algorithms \cite{putra2020analysis}, we present our adaptive job scheduling algorithm in Algorithm \ref{algo:adaptive-job-schedule}. This algorithm is designed to fulfill the aforementioned requirements as effectively as possible:

In {\em step 1.}, to maximize the fulfillment of objective \ding{186}, we employ a priority queue to rearrange jobs. They are sorted in descending order of priority. For jobs with the same priority, the one submitted earlier is placed at the front. In the next scheduling step, we select the top-k (where the user defines the parameter $top\_k$) jobs from the queue. Note that a job is removed from the queue only after its completion. In {\em step 2.}, we use Equation \ref{eq:memory-size} to estimate the resource requirements for each job among the top-k jobs. Then, by employing Equation \ref{eq:schedule-by-memory-size}, we can derive all feasible job scheduling methods that fulfill objective \ding{185}. In {\em step 3.}, using the predicted information, we estimate the number of iteration times needed to complete each job. Subsequently, we obtain the iteration time required for each job scheduling method. In {\em step 4.}, to maximize the fulfillment of objectives (\ding{182}\ding{183}\ding{184}), we employ the Shortest Job First (SJF) \cite{putra2020analysis} algorithm. 
%\Ye{in operation system this algorithm xxx}. 
This algorithm selects the scheduling method with the shortest time as the final scheduling result obtained from step 3.

During runtime, we optimize memory estimation and early stopping prediction models by collecting metric data through the profiler described in \S\ref{section:overview}. Any changes in memory estimation results and early stopping prediction results will initiate a re-scheduling action.

%\hspace{-1.3em}
%\Tang{example: }

==> OLDVER/OLDVER/chapters/VI._Experimental_Study.tex <==
%\vspace{-0.5em}
%In this section, we demonstrate the end-to-end performance of ASPEN and showcase the effectiveness of the adaptive scheduling algorithm.
%\vspace{-2.5em}
\subsection{Experimental Setup}

%\-\hspace{\parindent}
\textbf{Testbed.} In our experiments, we employed four distinct graphics cards: the NVIDIA GeForce RTX 4090 24GB~\cite{rtx4090}, NVIDIA RTX A6000 48GB~\cite{a6000}, and NVIDIA A100 80GB\cite{a100}. We used five diverse models: the LLaMA1~\cite{touvron2023llama} model with 7B and 13B parameters, the LLaMA2 model with 7B and 13B parameters, and the ChatGLM2~\cite{du2022glm} with 6B parameters.

%\smallskip
%\noindent\textbf{Simulator.} To assess the performance impact of various parameters on our adaptive scheduling algorithm across a large number of jobs, we developed a simulator, which utilizes information from traces collected during our testbed experiments, including memory utilization, completion time, and data size of jobs.

%\smallskip
\noindent\textbf{Workloads.} For training the LoRA model, we employed two public datasets: AlpacaCleaned\cite{alpaca} and Spider\cite{yu2019spider}. Each dataset obtained 90\% of its data for training through a sampling method.

%\smallskip
\noindent\textbf{Baseline.}
%As no existing system has implemented the sharing of pre-trained models for fine-tuning workloads, 
%\Tang{By following the previous model fine-tuning work Alpaca-LoRA~\cite{alpaca-lora},}
We set up the commonly used single-job LoRA fine-tuning system, i.e., Alpaca-LoRA~\cite{alpaca-lora}, as the baseline method. We compare system performance between ASPEN and using Alpaca-LoRA in two different ways. That is,  {\em Alpaca-Seq}: training models sequentially, one after another, on a single GPU; {\em Alpaca-Parallel}: concurrently training multiple models on a single GPU. We also compared the impact of four different scheduling strategies on the system: the \textit{MinPad} algorithm (name as $M3$) described in \S\ref{section:minpad}, FIFO scheduling algorithm (name as $M1$), priority scheduling algorithm (name as $M2$), and the adaptive scheduling algorithm (name as $M4$) described in \S\ref{section:adaptive-job-schedule}. 

%\smallskip
\noindent\textbf{Metrics.} The evaluation focuses on the following key metrics: 1) {\em Training Latency} or {\em Turnaround Time} ($TT$): representing the end-to-end time required for model training; 2) {\em Effective Throughput}: quantifying the number of tokens (excluding padding tokens) trained per second, providing insight into training process efficiency; 3) {\em GPU Memory Usage}: assessing the amount of memory allocated during the training process on the GPU; 4) {\em GPU Utilization Rate}: the workload processed by the GPU within a specified time period; 5) {\em Model Accuracy}: evaluating model performance using the MMLU accuracy score \cite{hendrycks2020measuring}; 6) {\em Waiting Time} ($WT$):  measuring the time spent waiting for the training job to start; 7) {\em Virtual Turnaround Time} ($VTT$): taking inspiration from the concept of virtual runtime in the Completely Fair Scheduler (CFS) algorithm \cite{kobus2009completely}, this metric is a normalized value of the real turnaround time, accounting for job priority. It is calculated as the product of the turnaround time and the priority, reflecting the accelerated virtual turnaround time for higher-priority jobs. For ease of representation, we normalized the time units and used $itime$ to denote time.

%\vspace{-3em}
\subsection{Performance Study}\label{sec:effective-throughput}
%%图片已上传
%\vspace{-0.5em}

In end-to-end performance experiments, we employed the same dataset to train four LoRA models with varying learning rates, monitoring the number of tokens and padding tokens trained per second and calculating the effective throughput and non-effective throughput. Figure \ref{fig:performance-compare} illustrates the results, where the \textit{Ineffective} portion represents non-effective throughput, and the others denote effective throughput. We compared (a) different models, (b) the same model architecture with different parameters and versions, and (c) the same model on different hardware. The training approach using ASPEN demonstrates a higher effective throughput by reducing kernel launch costs through {\em BatchFusion} operations and efficiently utilizing computational resources with job scheduling. The effective throughput has consistently improved by an average of 20\%.

%\smallskip
\noindent\textbf{Memory saving.}
%ASPEN can save pre-trained model weights; the saved memory can accommodate more LoRA modules for training. 
We compared the number of LoRA models that could be concurrently trained on a single A100 GPU using ASPEN and Alpaca-LoRA without encountering out-of-memory issues -- we gradually increased the number of jobs until triggering an out-of-memory situation while recording their memory usage. Figure \ref{fig:exp-mem} shows that with the batch size 2, ASPEN trains 6x as many concurrent LoRA modules as Alpaca-LoRA; with batch sizes of 4 or 6, this number is 3x; with a batch size of 8, it is doubled. In the scenario of concurrently training the same number of LoRA models, ASPEN can save an average of about 53\% of GPU memory compared to the approach without optimization.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{pics/join_picture.pdf}
    \caption{The throughput of (a) different models, (b) different parameters and versions, and (c) using different hardware.}
    \label{fig:performance-compare}
    %\vspace{-2em}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{pics/GPU_memory_usage.pdf}
    %\vspace{-1em}
    \caption{The GPU memory usage of Alpaca-LoRA and ASPEN with NVIDIA A100 80GB.}
    \label{fig:exp-mem}
    %\vspace{-1em}
\end{figure*}

%\smallskip
\noindent\textbf{System resource utilization.}
ASPEN can efficiently utilize GPU computational resources and reduce memory usage. 
%We collected data on GPU utilization and GPU memory usage per second. 
As shown in Figure \ref{fig:gpuutil}, ASPEN has an average GPU utilization 1\% higher than Alpaca-Parallel (with smaller fluctuations), while significantly reducing the average memory usage of jobs by sharing the pre-trained model. Thus, the job scheduling algorithm of ASPEN can effectively maintain GPU utilization at around 98\%.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.9\linewidth]{pics/Exp_loss.pdf}
%     \caption{The loss curves during the training of models with Alpaca-LoRA and ASPEN.}
%     \label{fig:exp-loss}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.9\linewidth]{pics/exp-acc.pdf}
%     \caption{The MMLU accuracy score of the models.}
%     \label{fig:exp-acc}
% \end{figure}

%When the loss value during training becomes abnormal (e.g., becomes $NaN$) or accuracy drops, we stop the model training. 
%\smallskip
\noindent\textbf{Early stopping.}
%Early stopping is a common method for saving end-to-end training latency. 
To illustrate the impact of early stopping, 
%we use the same dataset to train LoRA models with four different learning rates.
we analyze the latency and effective throughput of jobs using early stopping versus those without it.
As shown in Figure \ref{fig:exp-early-stoppting}, early stopping does not change the effective throughput, but saves end-to-end training latency: Both Alpaca-Parallel and ASPEN save 36\% of the training latency, as this method avoids waiting for all training data to be completed.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{pics/gpu-memory-utilization1.pdf}
    \caption{GPU utilization and memory usage.}
    \label{fig:gpuutil}
    %\vspace{-1em}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{pics/early_stop_and_original.pdf}
    \caption{The effect of early stopping.}
    \label{fig:exp-early-stoppting}
    %\vspace{-1em}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{pics/Exp-Adaptive.pdf}
    %\vspace{-1em}
    \caption{The effect of adaptive job scheduling.}
    \label{fig:exp-adaptive}
    %\vspace{-2em}
\end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{pics/stra_compare.pdf}
    \caption{The effect of scheduling strategies.}
    \label{fig:exp-stra_compare}
    %\vspace{-1em}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{pics/join-accuracy-and-loss.pdf}
    %\vspace{-1.5em}
    \caption{Loss curve and MMLU accuracy score under three different learning rates(LR): $\alpha=1\times10^{-4}$, $\beta=2\times10^{-4}$, $\gamma=5\times10^{-5}$.}
    \label{fig:exp-acc}
    %\vspace{-1.5em}
\end{figure}

%\smallskip
\noindent\textbf{Effectiveness of MinPad.}
To demonstrate the effectiveness of \textit{MinPad} scheduling strategies, we design the following experiments: we split the AlpacaCleaned and Spider datasets into eight subset datasets and trained eight LoRA models. Note that, Due to out-of-memory issues when training multiple models with LoRA-Parallel. We compare LoRA-Seq with \textit{MinPad} ($M3$) and two other common scheduling algorithms: FIFO ($M1$) and priority ($M2$). Figure \ref{fig:exp-stra_compare} shows that $MinPad$ improves the effective throughput by 21\% and reduces end-to-end training latency by 17\% compared to the baseline. However, for the other two scheduling strategies ($M1$ and $M2$), due to a lack of consideration of the padding issue, they result in 
a 30\% decrease in both latency and effective throughput.

%\smallskip
\noindent\textbf{Effectiveness of adaptive job scheduler.}
To validate the effectiveness of the adaptive scheduling algorithm in achieving improved system performance, we analyze its impact on throughput, turnaround time, waiting time, job priority, and memory management. The experiment involved the simultaneous submission of 100 jobs with varying execution times, memory requirements, and priorities.
These jobs underwent evaluation using three scheduling strategies: 
1) Priority Scheduling ($M2$),
2) $MinPad$ Scheduling ($M3$) and 
3) Adaptive Scheduling ($M4$).

Figure \ref{fig:exp-adaptive}(a) illustrates that the $MinPad$ strategy minimizes end-to-end time ($TT$). However, it compromises job priorities, reflected in an average virtual turnaround time ($VTT$) twice that of the priority scheduling algorithm. The Adaptive Scheduling Algorithm integrates the benefits of the shortest job first algorithm, reducing average turnaround time, average waiting time ($WT$), and end-to-end latency. Compared to the baseline, it achieves a 24\% reduction in turnaround time and a 12\% decrease in end-to-end latency while ensuring job priorities. The performance of the adaptive scheduling algorithm is affected by the user-defined top-k value and the accuracy of early stopping predictions. Figure \ref{fig:exp-adaptive}(d) shows that higher prediction accuracy correlates with reduced turnaround time. Figure \ref{fig:exp-adaptive}(b, c) indicates that increasing the top-k value decreases turnaround time, approaching the $MinPad$ algorithm's solution. However, this also entails a compromise on job priorities, as a smaller top-k value aligns the algorithm more closely with the priority scheduling approach, resulting in higher turnaround times.

%\smallskip
\noindent\textbf{Model convergence and performance.}
We trained three LoRA modules using the Alpaca-LoRA dataset and different learning rates with ASPEN and recorded the loss value for each iteration during the training process. Figure \ref{fig:exp-acc} (left side) shows that ASPEN and Alpaca-LoRA consistently ensure the convergence of model training. After training, we evaluated their accuracy score. As shown in Figure \ref{fig:exp-acc} (right side), the LoRA models trained by ASPEN exhibit accuracy almost identical to Alpaca, both about 2 points higher than LLaMA-7B. Thus, ASPEN does not affect the model's performance and ensures the training process converges as expected.
%\vspace{-2em}

==> OLDVER/OLDVER/draft/Draft_Algorithm.tex <==
\begin{algorithm}
    \caption{MinPad}
    \label{algo:minpad}
    \begin{algorithmic}[1]
        \Require Training Datasets: \textit{D}, The max fused-batch size: \textit{M}
        \Ensure Training fused-batch data: \textit{R}
        \State training dataset $d_\theta \gets random.pop(D)$
        \State training data $t_\alpha \gets random.pop(d_\theta)$ 
        \State training data set $l \gets empty()$ 
        \For{$d \in D$} 
        \State $t \gets find\_min(pad(t_\alpha, t \in d)) $
        \State $l \gets l \cup t$
        \EndFor
        \State $l.sort\_by(pad(t_\alpha, t \in l))$
        \State $R \gets FuseBatch(l.pop(M))$
    \end{algorithmic}
\end{algorithm}

==> OLDVER/OLDVER/draft/Draft_Intro.tex <==

%introduce the LLM fine tune and inference 
Large Language Models, commonly known as LLMs, have transformed the realm of natural language processing. Their immense capacity and generalization abilities have made them a cornerstone in various AI applications. While their raw capabilities are impressive, fine-tuning these models to specific tasks unlocks their true potential. Fine-tuning, a process wherein pre-trained LLMs are further trained on specific data to adapt to particular tasks, has become a popular approach to achieve high performance in numerous applications. Along with these unprecedented capabilities, generative LLM fine tuning comes
with unique challenges. These models can have billions, if
not trillions of parameters (Chowdhery et al., 2022; Fedus
et al., 2022), which leads to extremely high computational
and memory requirements to fine tune model. 


%introduce the motivation scenarios here
By leveraging the base model of the LLM during the processes of fine-tuning and inference, we showcase various applications of LLM optimized scenarios as below. 

\begin{itemize}
\item \textbf{Fine-tuning a LLM model on a single dataset with different hyperparameters can yield different outcomes}. By using the same foundational model as a base, researchers might experiment with various hyperparameters, such as adjusting the batch size, altering the learning rate, or employing different optimizers. Each combination can significantly influence the model's performance and adaptability to the specific dataset.

 \item \textbf{Fine-tuning LLM on multiple domain-related datasets allows for specialized domian applications}. For instance, one might adapt the model to legal datasets for a comprehensive understanding of jurisprudence, or further using healthcare data for medical expertise via fine-tune on patent-related datasets for insights into intellectual property. Regardless of the specific dataset, foundational models like Vicuna, LLMA2, or Llama serve as the shared basis for these specialized adaptations.

 %\item \textbf{LLM inference on multiple domains with shared-based model}. This shared foundation not only enhances their synergy but also opens avenues for them to collaboratively perform inference, thereby addressing complex challenges with a unified and harmonized approach.
\end{itemize}


%introduce the current shortage of Lora based approach. GPU memory usage shorage, utils, 
%introduce the previous fine tune work
Prior efforts to lower resource requirements of LLM fine tune correspond to three directions. Full parameter fine tuning, P-tunning, Q-tunning, xxx. 

%introduce the LORA based model fine tune 
By leveraging the mathematical properties of low-rank matrices, LoRA adapts pre-trained LLMs with a reduced parameter footprint, achieving effective fine-tuning without overwhelming computational costs.  

%introduce the major changgle here
To address these challenges, we present Apsen, an LORA fine tuning and inference framework for high-throughput LLM application. 

However, implement or design an effecient multi-lora framework for this senarises is not a trival work. For example, 1,2,3.  

% 1. offload 的策略算法？
% 2. 多任务的排队机制或者batch 机制？
% 3. Early stop 的多任务fine tune 优化？

Apsen aggregates memory from the GPU, CPU, and disk,
and efficiently schedules I/O operations, along with possible
compression methods and distributed pipeline parallelism. 


Overall, the major contribution of this work is summarized as below. 
\begin{itemize}
    % we build the multi
    \item We identify the challenges in batch and memory allocation in fine-tuning multiple
LLMs with shared based model and quantify their impact on fine tune performance.

    \item We propose a batch algorithm that operates on multiple jobs, which is inspired by the virtual memory and paging in OS, to improve the throughput. 
    
     \item We formally define a search space of
possible offloading and quantize strategies by considering computation
schedule, tensor placement, and computation delegation to reduce memory usage. 

    \item We evaluate vLLM on various scenarios and demonstrate
that it substantially outperforms the previous state-of-theart solutions such as .
\end{itemize}


==> OLDVER/OLDVER/draft/Draft_Opt.tex <==
\subsection{Problem Formulation}

\textbf{Memory Usage Analysis}: 

\textbf{Motivation:} \textit{is it possible to reuse the pre-trained weights to save the GPU memory?} If we perform $k$ training tasks with the same pre-trained weights, the theoretically percentage of GPU memory we can save is:

\begin{equation}
    \Delta_{\textit{shared-weights}} = \frac{(k-1)\Phi_P}{k\cdot\Pi}\%
\end{equation}

Our experimental validation on the NVIDIA RTX A6000 confirms our theoretical analysis: With a batch size of 8, sharing pre-trained models allows training more than twice the number of tasks simultaneously while consuming the same amount of memory.

% or GPU Utilization
\textbf{Computation Cost}: 
To assess the computational overhead, we conducted two fine-tuning tasks based on Alpaca-LoRA, running them serially\footnote{At any given moment, only one task is running, and another task is initiated only after the completion of the current one.} and in parallel\footnote{Two tasks start simultaneously, running asynchronously in two processes, using the same graphics card during the process.} on a single GPU. We then evaluated their throughput and average GPU utilization. The hyperparameter settings used in the experiment have been made publicly available on GitHub\footnote{https://github.com/yezhem/aspen-experiment}.

% 实验结果表明，无论是串行或是并行都无法完全利用单个GPU的全部算力。具体来看，在RTX A6000上并行运行两个任务的平均利用率提升了42%，吞吐量仅提升了14%；虽然在RTX 4090上并行运行两个任务的平均利用率提升了103%，高于RTX A6000，但吞吐量只提升了47%。

The experimental results indicate that both serial and parallel execution fail to fully utilize the entire computing power of a single GPU. Specifically, on the RTX A6000, running two tasks in parallel increased the average utilization by 42\%, but the throughput only increased by 14\%. While on the RTX 4090, running two tasks in parallel increased the average utilization by 103\%, surpassing the RTX A6000, the throughput only saw a 47\% improvement.

% 在两个不同GPU上进行的实验都表现出，当并行运行两个微调任务时，其增加的资源消耗与增加的吞吐量完全不成比例。也就是说，虽然并行运行微调任务会提升GPU的利用率，但也会造成更多的资源浪费。

The experiments conducted on two different GPUs both show that when running two fine-tuning tasks in parallel, the increased resource consumption is not proportional to the increased throughput. In other words, while parallel execution of fine-tuning tasks improves GPU utilization, it also leads to more resource wastage.

\begin{table}
    \centering
	\caption{Experiment to Evaluate Computation Cost} 
	\begin{tabularx}{\linewidth} {
        >{\raggedright\arraybackslash}X
        >{\centering\arraybackslash}p{3em}
        >{\centering\arraybackslash}p{6em}
        >{\centering\arraybackslash}X
        >{\raggedleft\arraybackslash}X
        }
		\hline 
		Method & Time & Throughput & Utilization & Memory \\
		\hline 
		S@A6000 & 6.23h & 505.03 token/s & 66.55\% & 9.44 GB \\
        P@A6000 & 5.47h & 575.75 token/s & 94.38\% & 18.87 GB \\
        S@4090  & 5.30h & 593.41 token/s & 37.72\% & 9.44 GB \\
        P@4090  & 3.60h & 874.39 token/s & 76.44\% & 18.87 GB \\
		\hline 
	\end{tabularx}
    \label{table:exp-comcost}
 \end{table}

Overall, we come to these conclusions:
\begin{itemize}
    \item Running multiple fine-tuning tasks serially does not effectively utilize resources;
    \item When running two fine-tuning tasks in parallel, the increased resource consumption is not proportional to the increased throughput;
    \item Parallel execution of fine-tuning tasks improves GPU utilization but also leads to more resource wastage.
\end{itemize}

Based on the analysis above, we believe that existing methods have not effectively utilized system resources. Thus, in this work, we focus on maximize system throughput and minimize training latency while satisfying the following constraints:
\begin{itemize}
    \item Does not trigger OOM\footnote{OOM: \textit{Out Of Memory}} error
    \item Ensure task priority
    \item Ensure the effect of fine-tuning
\end{itemize}


==> OLDVER/OLDVER/draft/III._Overview.tex <==


\subsection{ASPEN: A High-Throughput LLM Fine-Tuning Framework}

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{pics/Architecture.png}
    \caption{ASPEN System Overview}
    \label{fig:sys-overview}
\end{figure}

In this paper, we introduce a high-throughput large language model fine-tuning framework called \textbf{ASPEN}. This framework achieves parallel fine-tuning of multiple LoRA modules by sharing pre-trained model weights, thereby improving the efficiency of fine-tuning jobs on a single GPU. The architecture of ASPEN is illustrated in the Figure \ref{fig:sys-overview}, and its core involves a \textit{Job Coordinator} that dynamically allocates fine-tuning jobs based on system resources and user demands. The system mainly consists of three components:

\begin{enumerate}
    \item Job Coordinator: It dynamically selects a suitable set of jobs from the job pool by adjusting the priority coefficient, sequence coefficient, and affinity coefficient of jobs. It then uses the \textit{MinPad} algorithm to mitigate the negative impact on effective training throughput caused by aligning tokens;
    \item Multi-LoRA Trainer: This component employs the \textit{Batch Fusion} algorithm to merge training data from multiple fine-tuning jobs into a matrix, achieving parallel training on a single GPU with reduced GPU memory consumption and smaller computational overhead;
    \item Job Profiler: By monitoring various metrics such as Loss, Accuracy, GPU Utilization, GPU Memory, etc., this component provides feedback for the Job Scheduler's scheduling, supporting scheduling strategies like Early Stop based on job indicators.
\end{enumerate}

\subsection{Efficiently Sharing Pre-trained Model}

\begin{figure*}
    \centering
    \includegraphics[width=0.7\linewidth]{pics/ASPEN-LoRA.png}
    \caption{Multi-LoRA Method}
    \label{fig:multi-lora}
\end{figure*}

In this section, we introduce \textbf{Multi-LoRA} method, based on the LoRA approach, achieves more efficient reuse of pre-trained model weights during fine-tuning through Batch Fusion. The formula for $n$ jobs simultaneously undergoing fine-tuning is as follows:
\begin{align}
    H &= [W_0x_1 + \Delta W_1x_1,\ldots,W_0x_n + \Delta W_nx_n] \nonumber \\
    &= W_0X + [\Delta W_1x_1,\ldots,\Delta W_nx_n] \nonumber \\
    &= W_0X + [\Delta W_1,\ldots,\Delta W_n]X^T \label{eq:multi-lora}
\end{align}

Where $W_0 \in \mathbb{R}^{d \times k}$ is pre-trained weights, $\Delta W_i = B_iA_i$ is low-rank decomposition matrix for each job, $X$ is fused input batch.

\textbf{Holding Multiple Training Context}. It's easy to see that reusing pre-trained model weights can save a significant amount of GPU memory space. Since LoRA weights typically occupy minimal memory, is it possible to concurrently store multiple LoRA processes on a GPU?

We formulated the memory usage in the previous chapter. Taking LLaMA-7B as an example, the training process of one LoRA model requires approximately 44.5GB of GPU memory. Although checkpoint and gradient accumulation techniques are often used to save memory, holding multiple training contexts is still very challenging. However, if we share pre-trained weights using our method, it is not difficult to see that a significant amount of GPU memory can be saved. Assuming we perform $k$ training jobs with the same pre-trained weights, the theoretical percentage of GPU memory we can save is:

\begin{equation}
    \Delta_{\textit{shared-weights}} = \frac{(k-1)\Phi_P}{k\cdot\Pi}\%
\end{equation}

We validated this conclusion in our experiments: When the batch size is equal to 6, ASPEN can maintain twice the number of training jobs as existing methods by sharing pre-trained model weights.

Building on the above analysis, it is indeed feasible to concurrently store multiple LoRA training processes on a single GPU.

\textbf{Save Computation Cost}. GPU is a high-throughput computing device, and its characteristics determine that the computational cost of matrix operations is not strongly correlated with its size. Therefore, on a GPU, performing operations on a large matrix is often faster than on multiple small matrices. Inspired by the idea of operator fusion, we find that by fusing the training data of n fine-tuning jobs into a large matrix and multiplying it with shared pre-trained model weights, computational resources can be saved.

Assuming there are n jobs undergoing fine-tuning simultaneously, each matrix operation costing v, according to the LoRA formula, the computational cost is approximately 3n. However, in the Multi-LoRA method, based on formula X, the computational cost is approximately 2n. This makes our method 10\% faster than the LoRA approach. We validated this conclusion in our experiments.

\textbf{Padding Training Data}. Dealing with uneven lengths of training data from different fine-tuning jobs during the Batch Fusion process often requires the insertion of special tokens for alignment to ensure consistent dimensions for matrix composition. However, the presence of alignment tokens in the matrix is meaningless and can reduce effective training throughput. Mitigating the impact of alignment tokens on effective training throughput is not a trivial job.

Reducing the impact involves optimizing the token insertion strategy, perhaps by strategically placing alignment tokens only where necessary or by exploring advanced padding techniques. It requires a careful balance between achieving alignment and minimizing the introduction of unnecessary tokens to maintain efficient training throughput. This optimization process is often job-specific and may require experimentation to find the most effective approach.

\subsection{Reduce Negative Effect of Padding Tokens}

In this section, we propose the \textit{MinPad} algorithm to reduce the impact on effective training throughput by finding a set of training data that requires minimal padding in a fixed training job.

\begin{algorithm}
    \caption{MinPad}
    \label{algo:minpad}
    \begin{algorithmic}[1]
        \Require Training Datasets: \textit{D}, The max fused-batch size: \textit{M}
        \Ensure Training fused-batch data: \textit{R}
        \State training dataset $d_\theta \gets random.pop(D)$
        \State training data $t_\alpha \gets random.pop(d_\theta)$ 
        \State training data set $l \gets empty()$ 
        \For{$d \in D$} 
        \State $t \gets find\_min(pad(t_\alpha, t \in d)) $
        \State $l \gets l \cup t$
        \EndFor
        \State $l.sort\_by(pad(t_\alpha, t \in l))$
        \State $R \gets FuseBatch(l.pop(M))$
    \end{algorithmic}
\end{algorithm}

\textbf{Uneven Distributed Training Data.}
In practice, the lengths of most datasets roughly follow a Poisson distribution. Taking the commonly used AlpacaCleaned dataset as an example, its data length distribution is shown in the graph. When multiple jobs with different datasets are trained in parallel, the training data lengths vary in each iteration. In experiments, when using our proposed Batch Fusion method without applying any optimization strategy, aligning tokens can occupy up to 30\% of the total token count, resulting in an effective throughput of only around 85\% of the total throughput of the entire training process.

\textbf{Optimization Strategies.} 
AlpacaLoRA uses \textit{Group By Length} to solve this problem, while it can only solve the problem inside each batch of jobs. Our approach not only takes into account the training data distribution for each job but also includes all jobs waiting for training in the candidate set. This significantly expands the algorithm's search space, further reducing the number of aligned tokens on top of the Group By Length approach. In the experiments, the effective throughput of ASPEN after applying the MinPad algorithm is 10\% higher than AlpacaLoRA with \textit{Group By Length} enabled, reaching 600 tokens/s.

\textbf{Limitations of MinPad.}
The core idea of the MinPad algorithm is to seek the global optimal solution for the optimization problem of minimizing misaligned tokens across all known training jobs. However, this approach tends to overlook job priorities, leading to a longer average job turnaround time. Moreover, practical application scenarios often involve dynamic changes in the number of jobs. Balancing the benefits of the MinPad algorithm with the requirements of real-world applications is a non-trivial job.

\subsection{Job Coordination}

In this section, we introduce the Job Coordination algorithm, aiming to integrate job priority, order, and affinity. This integration facilitates a sensible allocation of job resources, taking into account both system resources and user needs.

==> OLDVER/OLDVER/draft/IV._Optimization.tex <==
In this chapter, we propose \textit{Multi-LoRA} to address the issue of sharing pre-trained weights introduced in Chapter 3. The architecture of Multi-LoRA is illustrated in Figure \ref{fig:multi-lora}. Inspired by the concept of operator fusion, Multi-LoRA fuses multiple input matrices into a larger matrix before training to reduce the cost. 

Next, we observe that the valid training throughput is affected by the number of extra alignment tokens introduced due to the variable length of input data. We introduce the \textit{MinPad} Algorithm to minimize the impact of extra alignment tokens.

Finally, when the number of tasks can be determined before training, the \textit{MinPad} Algorithm can produce a global optimum that achieves maximum valid training throughput by reducing the impact of alignment tokens. However, it may also lead to a longer turnaround time for tasks. Based on these considerations, we propose a scheduling algorithm with a sliding window to address this issue.

\subsection{Reusing Pre-trained Weights}

The Multi-LoRA method is built upon original LoRA\cite{hu2021lora}, achieving the reuse of pre-trained model weights and reducing computational costs by fusing input data from multiple fine-tuning tasks into a large matrix.

\textbf{Motivation.} As described in Equation \ref{eq:lora}, the forward pass of LoRA is very straightforward. Assuming we have $n$ training tasks running at the same time, the forward pass of all tasks is as follows:
\begin{align*}
    h_1 &= W_0x_1 + \Delta W_1x_1 \\
    h_2 &= W_0x_2 + \Delta W_2x_2 \\
    &\cdots \\
    h_n &= W_0x_n + \Delta W_nx_n
\end{align*}

Where $W_0$ represents frozen pre-trained weights, $h_i$ is the output matrix, $x_i$ is the input matrix at the current iteration, and $\Delta W_i = B_iA_i$ is the low-rank parameter update matrix. It's evident that in the computation process of $h_1, \ldots, h_n$, the reuse of $W_0$ can be achieved by a serial operation, such as foreach loops. PEFT\cite{peft} has already implemented this approach. However, as analyzed in Chapter 3, serial computation cannot effectively utilize the GPU's resources.

\textbf{Matrix Fusion.} Inspired by the idea of operator fusion, we fuse $x_1, \ldots, x_n$ into a large matrix $X$ before computation. Therefore, the computation formula can be transformed into:
\begin{align}
    H &= [W_0x_1 + \Delta W_1x_1,\ldots,W_0x_n + \Delta W_nx_n] \nonumber \\
    &= W_0X + [\Delta W_1x_1,\ldots,\Delta W_nx_n] \nonumber \\
    &= W_0X + [\Delta W_1,\ldots,\Delta W_n]X^T \label{eq:multi-lora}
\end{align}

In this simplified formula, the pre-trained model weights are multiplied in a single operation with the fused input matrix $X$, while subsequent multiple $\Delta W$ multiplications with the transpose of $X$ can be executed in parallel. Therefore, based on Formula \ref{eq:multi-lora}, we can achieve weight sharing of pre-trained models among parallel LoRA tasks with lower extra overhead.

\textbf{Memory Usage Analysis.}

\textbf{Computation Cost Analysis.}
To simplify the analysis of the model, we assume that a matrix operation process will launch one CUDA kernel, and the cost of each kernel launch is $\sigma$. According to the computation process of $h_1, \ldots, h_n$, the computation cost of the trivial approach is:
\begin{equation}
    \Theta_{\textit{parallel}} = 3n\cdot\sigma \label{eq:cost-trivial}
\end{equation}

In Multi-LoRA, we fuse $x_1, \ldots, x_n$ into a large matrix $X$ before computation. Therefore, the computation cost of our approach is:
\begin{equation}
    \Theta_{\textit{fusion}} = (2n + 1)\cdot\sigma \label{eq:cost-aspen}
\end{equation}

According to Formula \ref{eq:cost-trivial} and \ref{eq:cost-aspen}, we can easily deduce that Multi-LoRA can save approximately $n\cdot\sigma$ computation cost per forward pass compared to the trivial approach. Our ablation experiment shows that the forward pass of Multi-LoRA is 30\% faster than the parallel execution of Alpaca-LoRA.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{pics/Fig-Padding.png}
    \caption{Matrix Alignment Based on Special Tokens}
    \label{fig:padding}
\end{figure}

\subsection{Minimal Alignment Tokens}
The training data lengths for each task are various. To merge these varying-length training data into a single matrix, special tokens need to be used for aligning the rank of the matrices. However, as shown in Figure \ref{fig:padding}, these special alignment tokens are meaningless and can decrease effective training throughput.

% 增加示例分析为什么会影响吞吐量
% 增加模拟实验，算出实际影响因子

To address this issue, we propose the MinPad Algorithm, which seeks a set of data with the minimum number of alignment tokens for training among the $n$ tasks with a fixed quantity. This minimizes its impact on effective training throughput.



% 增加示例分析算法原理

\subsection{High Throughput Scheduling}

% 目标：低周转时间、高吞吐量、保证优先级
% 方法：资源预估、优先队列、综合（ = 优先系数 + 顺序系数 + 亲和系数，取前j个）

The overall approach of the scheduling algorithm in Multi-LoRA involves incorporating a sliding window onto a FIFO queue and applying the MinPad algorithm within the window's scope. This reduces the impact of alignment tokens on effective training throughput while decreasing the average turnaround time for tasks.

\textbf{Motivation.} 
In the previous section, we observed that in our approach, the quantity of special tokens used for alignment in the input data significantly affects training throughput. Choosing a subset of data with the minimum number of alignment tokens from multiple training tasks can mitigate this issue. The MinPad Algorithm is designed based on this concept. While pursuing a global optimum from all training tasks achieves optimal performance, it introduces two challenges:
\begin{enumerate}
    \item The pursuit of a global optimum is contingent upon the determination of the training task set. Our approach enables the dynamic inclusion and exclusion of training tasks, thereby rendering the notion of a global optimum untenable;
    \item If pursuing a global optimum, it also may result in tasks added later finishing earlier than those added first, leading to a longer average turnaround for tasks.
\end{enumerate}

\textbf{Limiting the Search Space.} We employ a first in and first out(FIFO) queue and utilize a sliding scheduling window to limit the search space of the MinPad Algorithm, which means a new training task will be introduced only after the completion of the first task within the window. The modified scheduling procedure is depicted in Algorithm \ref{algo:optimal-minpad}.

In this scheduling queue, the count of parallel tasks $n_p$ specifies how many tasks are included in the fused batch, and the sliding window size $n_w$ specifies the search range of the MinPad algorithm. To save memory, we will only load tasks within the window range into memory, thereby avoiding unnecessary resource usage.

Overall, this mechanism reduces the average turnaround time of tasks by limiting the search space of the algorithm. At the same time, it allows for the dynamic variation in the number of training tasks, providing greater flexibility in the training schedule.

\begin{algorithm}
    \caption{MinPad}
    \label{algo:minpad}
    \begin{algorithmic}[1]
        \Require Traning Datasets: \textit{D}, The max fused-batch size: \textit{M}
        \Ensure Traning fused-batch data: \textit{R}
        \State Get $\textit{d}_\theta$ from \textit{D} randomly, $\textit{D} \gets \textit{D} - \textit{d}_\theta$
        \State Get $\textit{t}_\alpha$ from $\textit{d}_\theta$ randomly, $\textit{d}_\theta \gets \textit{d}_\theta - \textit{t}_\alpha$
        \State Iinitialize Priority queue $\textit{Q}$
        \For $\textit{d} \in \textit{D}$
        \State xx
        \EndFor
    \end{algorithmic}
\end{algorithm}

==> OLDVER/OLDVER/draft/IV._Optimization_Strategies.tex <==
%\textbf{Multi-Lora Optimization}

In this section, we introduce major three components in this work. that is ...

\subsection{Multi Jobs Batch Auto Padding}




\subsection{Throughout Oriented Job Scheduling}





%\subsection{Fast Job Batching}



==> OLDVER/OLDVER/draft/V._Discussion.tex <==
The training cost of large language models is very high, especially professional computing cards with high memory capacity (such as NVIDIA Quadro) are very expensive. For small scientific research teams, consumer-grade graphics cards such as NVIDIA RTX 4090 are often more cost-effective. However, although these computing cards can compete with professional computing cards in terms of computing power, they often have smaller video memory, which limits the demand for higher video memory. Computational tasks, this is especially obvious in the fine-tuning task of large language models.

The common practice in the industry is to use Offloading and Quantization to solve the problem of limited video memory. For example, DeepSpeed uses ZeRO-Offload\cite{rajbhandari2021zeroinfinity} to optimize video memory usage, and QLoRA\cite{dettmers2023qlora} uses 4bit quantization to fine-tune a 65B model on a 48G graphics card. In our application scenario, unnecessary graphics memory overhead caused by multiple base models has been saved, but there are still many restrictions on consumer-grade graphics cards; and because multiple models are fine-tuned at the same time, there will be video memory There is a problem of being idle but not able to accommodate another training task, which will limit the GPU throughput to a certain extent.

Multi-LoRA supports 8-bit and 4-bit quantization based on Bitsandbytes\cite{dettmers2022llmint8}, allowing users to freely configure according to usage scenarios; based on PyTorch Autograd, Offload is implemented based on Checkpoint, which will be introduced in detail in next section.

\subsection{Offloading}

The algorithm used by Multi-LoRA to implement Offloading is based on checkpoint, that is, hooks are inserted into the pack and unpack processes of checkpoints, and unused checkpoints will be temporarily transfer to system memory. When transferring, Multi-LoRA will only save the forward data, masks, state amount when calculating attention, and input data of each layer, thereby reducing overhead as much as possible. In order to quantitatively analyze the cost of offloading, we established cost models for the two strategies of offloading and recompute. Assuming that the function $b(\textit{device})$ is the bandwidth of the computing device, $w$ is the constant of the time it takes for the system to load and restore state, the objective functions are:

\begin{equation}
    \label{offloading_obj}
    T_{\textit{offloading}}=\frac{2\times\textit{layer.count}\times \textit{layer.size}}{\textit{min}(b(\textit{mem}),b(\textit{vMem}),bw(\textit{pcie}))}
\end{equation}

\begin{equation}
    \label{recompute_obj}
    T_{\textit{recompute}}=\textit{layer.count}\times(\frac{2\times \textit{layer.size}}{b(\textit{vMem})}+w)
\end{equation}

When the number of layers and the amount of data to be saved in each layer are constant, the cost of offloading is mainly limited by the PCI-E bandwidth, which is often less than one-twentieth of the memory bandwidth\footnote{PCIE 4.0x16 = 32GB/s, GDDR6X 384bit = 1TB/s}. In this case, the overhead of offloading will be more than 10 times that of the optimal case of recompute. In practice, because the backward of the model takes up a large part of the running time, the cost of offload is only about 1.2 times that of recompute.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{pics/4.3.1.png}
    \caption{Async Offloading Prefetch time consumption compared with other methods}
    \label{fig:async-offloading}
\end{figure}

The main problem at present is that the method we use to implement Offload (PyTorch Autograd) can only trigger Offload synchronously on-demand. If the timing of Offload can be accurately controlled, as shown in Figure \ref{fig:async-offloading}, the Async Offloading Prefetch of the $N+1$ layer is automatically triggered when Recompute starts at the layer $N$, and then by analogy, higher efficiency can be achieved than simple recompute.

\subsection{Early Stop}

The two methods mentioned above improve GPU utilization without affecting the training task itself as much as possible, but in actual applications, not every task is worth occupying precious computing power. To solve this problem, a common practice in the industry is Early Stop (insert related work introduction here). There are many indicators for Early Stop, such as Loss, Prediction Precision and Recall, etc. Loss is not very commonly used in the training process of large language models, because a lower Loss value may represent overfitting and cannot better represent the training results of the model; prediction Precision and Recall are relatively accurate, and there are many evaluation methods. Such as (related work), but it can only reflect the effect of large language models in zero-shot or few-shot tasks, and it is difficult to evaluate its core reasoning capabilities; (insert other related work here).

In order to apply Early Stop to save computing power, Multi-LoRA reserves relevant interfaces during the training process, allowing the scheduler to evaluate the checkpoint of the model in real time.

==> OLDVER/OLDVER/draft/VI._Implementation.tex <==
\subsection{LLaMA Model}
A LLaMA compatible model is based on Transformer\cite{vaswani2023attention} architecture composed by normalization layer and certain transformer layer\cite{touvron2023llama}. To achieve the goal of optimizing the entire Multi-LoRA workflow, we re-implemented the entire LLaMA architecture, diverging from the common practice of making improvements on the foundation of HuggingFace's work, as is typically done.

However, to maintain support for mainstream models, we still implemented model loading using the \textit{LlamaForCausalLM.from\_pretrained} method from the HuggingFace's Transformers library\cite{wolf2020huggingfaces}. Additionally, we implemented quantization for both 8-bit and 4-bit based on the Bitsandbytes approach\cite{dettmers2022llmint8}.

The computation of the model primarily consists of two processes: forward and backward. In our implementation, we concentrated on implementing the model's forward process, while relying on PyTorch's Autograd to automatically generate the backward process. To conserve unnecessary GPU memory consumption, we employed checkpoints to optimize memory usage, incorporating two strategies: recomputation and offload. Due to the higher overhead associated with Offload (as elucidated in the discussion section), we default to using recomputation.

\subsection{Transformer Layer}

Following the architecture and formulas of the Transformer, we implemented the $Q, K, V, O$ modules in the attention layer, as well as the $W_1, W_2, W_3$ in the fully connected layer, using linear layers (as will be discussed in the next section). Additionally, we incorporated the RMSNorm normalization layer\cite{zhang2019root} based on the LLaMA paper.

\subsection{Linear Module}

As mentioned earlier, we completely re-implemented the entire LLaMA model along with the Transformer layer, but did not elaborate on how we achieved simultaneous fine-tuning or inference of multiple LoRA modules. In practice, to simplify the implementation, we encapsulated this logic within the Linear layer. During the loading process, different LoRA weights are decomposed into various Linear layers based on $Q, K, V, O, W_1, W_2, W_3$. Then, in the forward pass of the model, as illustrated in Figure \ref{fig:multi-lora} at the beginning of the paper, we first pass the entire batch of data through the Linear weights of the base model. Subsequently, we decompose the batch and simultaneously pass it through the corresponding weights of each LoRA module. Finally, we sum the results into a large matrix, which is then passed to the trainer. Full forward pass are described in Algorithm \ref{algo:linear-module}.

\begin{algorithm}
    \caption{Linear Module Forward}
    \begin{algorithmic}[1]
        \Function{Forward}{$base,loras,data,args$}
        \Comment{$base$ is weights of base model, $loras$ is weights of LoRA models, $data$ is input batch tensor; $args$ contains batch configurations.}
        \State $T\gets base.forward(data)$
        \For{$config\in args.batch\_configs$}
        \State $BeginCudaStream()$
        \State $M\gets loras[config.name]$
        \State $D\gets data[config.data\_range]$
        \State $T\gets T+M.forward(D)$
        \State $EndCudaStream()$
        \EndFor
        \State $CudaSynchronize()$
        \State \Return $T$
        \EndFunction
    \end{algorithmic}
    \label{algo:linear-module}
\end{algorithm}

\subsection{Checkpoints}

\textit{TO BE FILLED BY Ye}

\subsection{Dispatcher}

\textit{TO BE FILLED BY Ye}


==> OLDVER/OLDVER/draft/draw_draft.tex <==
\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{0.4\linewidth}
        \includegraphics[width=\linewidth]{pics/revise_llma_compare.pdf}
        \caption{Different LLaMA1}
        \label{fig:llama-compare}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.2\linewidth}
        \includegraphics[width=\linewidth]{pics/revise_qlora_compare.pdf}
        \caption{Caption for QLoRa}
        \label{fig:qlora-compare}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\linewidth}
        \includegraphics[width=\linewidth]{pics/revise_device_compare.pdf}
        \caption{Caption for Device Comparison}
        \label{fig:device-compare}
    \end{subfigure}
    \caption{Overall caption for all three figures}
    \label{fig:overall-figure}
\end{figure}


==> OLDVER/OLDVER/draft/exp.tex <==
\section{Draft Exp}

\textbf{Training Multiple LoRA Modules.} In this workload, we conducted four identical fine-tuning jobs with the XXX dataset and a batch size of N in NVIDIA RTX A6000, incorporating two baselines and ASPEN. During the experimental process, we collected the completion times for each task in the baseline methods and calculated the time taken by the slowest task as the \textit{Training Latency}. As shown in Figure \ref{fig:timecost}, ASPEN exhibits lower \textit{Training Latency} compared to both baseline methods. Specifically, ASPEN is 9.99\% faster than Baseline@SEQ and 3.92\% faster than Baseline@SYNC.

While ASPEN demonstrated significantly superior performance to the baseline methods in the above experiments, it is common in practical applications to employ Early Stop to terminate underperforming tasks, thereby avoiding resource waste. To align more closely with real-world scenarios, we applied Early Stop on top of the aforementioned experiments.

\textbf{Applying Early Stop Strategy.} In this workload, we reused the experimental settings mentioned above but applied the early stop strategy based on loss for tasks. As depicted in Figure \ref{fig:timecost}, the Training Latency for all three methods significantly decreased. However, ASPEN remains the optimal method, further widening the gap with the baselines. Specifically, ASPEN is 14.87\% faster than Baseline@SEQ and 9.36\% faster than Baseline@SYNC.


\subsection{Memory Usage Analysis}


\subsection{Effect of Job Scheduling}


\subsection{Ablation Studies}

\textbf{Batching}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{pics/Exp-Batch.pdf}
%     \caption{Experimental results of ASPEN's three different batch strategies and baseline methods in terms of latency, throughput, memory utilization, and GPU utilization. \textit{We need to use padded throughput and actual throughput to illustrate the benefit of our sequence scheduling method}}
%     \label{fig:batchtest}
% \end{figure}


In Chapter IV, an elaborate discussion was conducted on two distinct batch strategies, namely Optimal-Fit and Fast-Fit. Varied impacts on training arise from the adoption of these different strategies. To enable the selection of the most suitable batch strategy for diverse requirements, we configured two distinct sets of hyperparameters for the previously mentioned four datasets, thereby constituting eight distinct training tasks for experimentation.

As shown in Figure \ref{fig:batchtest}, \textit{M1, M2, M3} represent three batch strategies: Optimal-Fit, Trivial, and Fast-Fit, respectively. \textit{BASELINE} denotes the baseline method of sequential execution. The Optimal-Fit strategy performs the best across all four metrics, while the other two strategies also outperform the baseline method.

\textbf{Max Parallel Tasks in Different Batch Size}



Batch Size is a critical parameter in training, as it is not only positively correlated with GPU memory consumption but also exerts a certain degree of influence on training efficacy. To investigate the divergent impacts of different Batch Sizes on both the baseline method and ASPEN, we progressively increased the number of training tasks on a single GPU for Batch Sizes of 4, 6, and 8 until encountering an Out-Of-Memory (OOM) event.

Figure \ref{fig:memtest} shows the peak memory usage of the existing method compared to our method on one NVIDIA RTX A6000 GPU with batch size = 4, 6 and 8. The existing method triggered an OOM error after 3 parallel tasks when batch size = 8, while our method can handle twice that amount.

\textbf{Performance of Forward and Backward}

From the preceding experiments, we observed that ASPEN outperforms the baseline method in both latency and throughput. To further enhance performance, we collected the time consumption data for the Forward and Backward processes of ASPEN and the baseline method separately.

The results indicate that ASPEN's Forward process is significantly faster than the baseline method. However, the Backward process is somewhat slower, attributed to ASPEN feeding input data from multiple LoRA modules to the base model in a single batch, thus better leveraging the GPU's computational power. Nevertheless, the Backward process, relying on PyTorch Autograd, does not match the efficiency of manually optimized methods. Our next step involves optimizing the Backward process to address this issue and further enhance overall performance.

\textbf{Performance with Different Base Model}

Experiment on 7B and 13B

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.9\textwidth]{pics/join_picture.pdf}
%     \caption{caption}
%     \label{fig:performance-compare}
% \end{figure*}

\textbf{Performance with Different Quantization}

Experiment on 8bit and 4bit

Various GPU architectures, the number of streaming multiprocessors (SMs), memory bandwidth, and other factors can significantly impact the performance of fine-tuning. To ensure that ASPEN achieves favorable results across a range of mainstream GPUs, we conducted tests on two professional-grade graphics cards (A6000, A5000) and two consumer-grade graphics cards (RTX 4090, RTX 3090).
